Less is More: Multimodal Region Representation via Pairwise Inter-view Learning

With the increasing availability of geospatial datasets, researchers have explored region representation learning (RRL) to analyze complex region characteristics. Recent RRL methods use contrastive learning (CL) to capture shared information between two modalities but often overlook task-relevant unique information specific to each modality. Such modality-specific details can explain region characteristics that shared information alone cannot capture. Bringing information factorization to RRL can address this by factorizing multimodal data into shared and unique information. However, existing factorization approaches focus on two modalities, whereas RRL can benefit from various geospatial data. Extending factorization beyond two modalities is non-trivial because modeling high-order relationships introduces a combinatorial number of learning objectives, increasing model complexity. We introduce Cross modal Knowledge Injected Embedding, an information factorization approach for RRL that captures both shared and unique representations. CooKIE uses a pairwise inter-view learning approach that captures high-order information without modeling high-order dependency, avoiding exhaustive combinations. We evaluate CooKIE on three regression tasks and a land use classification task in New York City and Delhi, India. Results show that CooKIE outperforms existing RRL methods and a factorized RRL model, capturing multimodal information with fewer training parameters and floating-point operations per second (FLOPs). We release the code: https://github.com/MinNamgung/CooKIE.

==> backup/experiments.tex <==
\section{Experiments}
We evaluate \modelname by using the learned region embeddings to predict population density, crime rates, land use classification, and greenness. The first three are common downstream tasks in region representation, and greenness is an important indicator for public health, as a proxy for measuring environmental quality and well-being~\cite{dronova2018spatio, green}. We test these downstream tasks in New York City (NYC) and Delhi, India, where the size of geographic partitions varies. 

\subsection{Datasets} 
\subsubsection{POIs ($\mathcal{P}$) and AOIs ($\mathcal{A}$).}
We extract POI and AOI features from OpenStreetMap (OSM) and aggregate them into 27 predefined categories for POI and 34 for AOI~\cite{zhao2023learning}.
For OSM types that do not correspond to the existing categories, we establish additional categories to ensure a comprehensive classification. 
% We use $\mathcal{P}$ as POI and $\mathcal{A}$ as AOI. 

\subsubsection{Satellite Imagery ($\mathcal{S}$).}
For NYC, we collect satellite imagery from the National Agriculture Imagery Program (NAIP) with a spatial resolution of 1 meter in 2021. For Delhi, we collect data from PLANET with a spatial resolution of 3 meters in 2023. 
% Since regions vary in size, satellite imagery also differs in scale across regions.
To standardize the size of satellite images across regions and enhance the diversity of regional aspects, we preprocess neighborhood-level images using a patching method for those large satellite imagery.
We first divide the image into multiple patches and then randomly select and combine these patches into a single image for the image size is much larger than the standard size. 
% Additionally, we apply a cropping method for images with one disproportionately large side to refine the image further.
For images with one disproportionately large side, we apply a cropping method to adjust them to the standard size.
% For one side of the image is large, we apply a cropping method for images with one disproportionately large side to become the standard size. 
This approach helps capture diverse features and details within each region. 

\subsubsection{Building Footprints ($\mathcal{B}$).} 
We obtain 2D polygonal building footprint data from OSM in NYC and Delhi. 

\subsubsection{Downstream Tasks}
For NYC, we collect population density from WorldPoP\footnote{\url{https://hub.worldpop.org/geodata/listing?id=77}}, land use data from NYC MapPLUTO\footnote{\url{https://www.nyc.gov/site/planning/data-maps/open-data/dwn-pluto-mappluto.page}}, crime data from NYC Open Data\footnote{\url{https://opendata.cityofnewyork.us/}}, and the greenness indicator from Treepedia~\cite{green}. 
For Delhi, we generate the greenness scores following the procedure in~\cite{green}. Specifically, we query Google Street View images at road intersections, covering four directions, and perform semantic segmentation using OneFormer~\cite{oneformer}, fine-tuned with the Cityscapes dataset~\cite{cityscapes}. Then we compute the greenness score as $\text{Greenness} =\frac{\sum_{i=1}^4Area_{g}}{\sum_{i=1}^4Area_{a}}$ for each intersection, where $Area_{g}$ represents the number of green pixels in the image and $Area_{a}$ is the total number of pixels.
Finally, we take an average of the greenness score for each ward to generate the greenness indicator for Delhi. 
% \begin{figure}[h]
% \vspace{-0.8em}
% \setlength{\belowcaptionskip}{-9pt}
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/gvi_nyc_V2.png}
%         \caption{New York City}
%         % \vspace{-2em}
%         \label{gvi_nyc}
%     \end{subfigure}
%     % \vspace{2em}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/gvi_delhi.png}
%         \caption{Delhi}
%         \label{gvi_delhi}
%         % \vspace{-2em}
%     \end{subfigure}
%     \caption{Greenness Distribution}
%     \label{gvi_fig}
%     \hfill
% \end{figure}
% Figure~\ref{gvi_fig} visualizes the greenness indicator in NYC and Delhi. Notably, the boundary sizes of regions and the completeness of data vary between the two cities.

\subsection{Baselines}
We compare \modelname to seven state-of-the-art methods, grouped into inter-view only and intra- \& inter-view learning: 
\subsubsection{Inter-view only}
\begin{itemize}
    \item MVURE~\cite{mvure} utilize $\mathcal{P}$ and human mobility ($\mathcal{M}$) in a graph attention network, where each node represents a region and each edge represents a connectivity between two regions. We exploit the learned embeddings from RegionDCL~\cite{li2023urban}.
    \item KnowCL~\cite{liu2023knowledge} combines a knowledge graph ($\mathcal{KG}$) and geospatial visual features in inter-view contrastive learning, with the knowledge graph based on spatial location, $\mathcal{P}$, and $\mathcal{M}$. In Table~\ref{table_result_1}, the ($\log$) notation indicates that a 1-fold train-test split was used, and the labels were transformed to a logarithmic scale, $y = \ln(y_{raw} + 1)$.
    % the indication of ($\log$) represents that the evaluation is performed with a 1-fold train-test split, and the labels were transformed into a logarithmic scale, (i.e., $y = ln(y_{raw} + 1)$)~\cite{liu2023knowledge}. 
    \item FactorCL~\cite{factorcl} is extended to learn unique and shared information among three modalities.
\end{itemize}
\subsubsection{Intra- \& Inter-view learning}
\begin{itemize}
    \item MGFN~\cite{wu2022multi_mgfn} identifies mobility patterns and learns representation by self-attention mechanism. We use the embedding from RegionDCL~\cite{li2023urban}.
    \item RegionDCL~\cite{li2023urban} combines building footprints and $\mathcal{P}$ with a contrastive learning approach by considering building group and regional levels. We feed $\mathcal{B}$, $\mathcal{P}$, and $\mathcal{A}$ to train the model.
    \item Urban2Vec~\cite{wang2020urban2vec} fuses street view imagery and $\mathcal{P}$ description from Yelp reviews using triplet loss. We feed $\mathcal{S}$ and textual data (names and types) describing $\mathcal{P}$ and $\mathcal{A}$. 
    \item ReMVC~\cite{tkde} learns distinctive region features by intra-view learning and captures mutual information in inter-learning through contrastive learning. We use the three modalities ($\mathcal{P}$, $\mathcal{A}$, $\mathcal{S}$) as inputs with $\mathcal{P}$ and $\mathcal{A}$ concatenated before feeding them into ReMVC.
\end{itemize}

% \begin{itemize}
%     \item Urban2Vec~\cite{wang2020urban2vec} fuses street view imagery and POI description from Yelp reviews using triplet loss. We feed satellite imagery and textual data (names, types) describing POIs and AOIs. 
%     \item MVURE~\cite{mvure} combines POIs and human mobility in a graph attention network. We exploit the learned embedding from RegionDCL~\cite{li2023urban}.
%     \item MGFN~\cite{wu2022multi_mgfn} identifies mobility patterns and learns representation by self-attention mechanism. We use the embedding from RegionDCL~\cite{li2023urban}.
%     \item KnowCL~\cite{liu2023knowledge} integrates knowledge graph and geospatial visual features in inter-view contrastive learning. The knowledge graph is built upon spatial location, type, POIs, and mobility data.
%     \item RegionDCL~\cite{li2023urban} combines building footprints and POIs with a contrastive learning approach by considering building group and regional levels. We feed building footprint, POIs, and AOIs to train the model.
%     \item FactorCL~\cite{factorcl} capture unique and shared information in multiple modalities. We test the extension version of FactorCL by feeding the same three inputs as \modelnamex.
%     \item ReMVC~\cite{tkde} learns intra- and captures mutual information in inter-learning through contrastive learning. We use the same three modalities (POI, AOI, SAT) as inputs, with POI and AOI concatenated before feeding them into the model.
% \end{itemize}


% We compare \modelname to six state-of-the-art region representation baseline models.
% \begin{itemize}
%     \item Urban2Vec~\cite{wang2020urban2vec} fuses street view imagery and POI description from Yelp reviews using triplet loss. We feed satellite imagery and textual data (names, types) describing POIs and AOIs. 
%     \item MVURE~\cite{mvure} combines POIs and human mobility in a graph attention network. We exploit the learned embedding from RegionDCL~\cite{li2023urban}.
%     \item MGFN~\cite{wu2022multi_mgfn} identifies mobility patterns and learns representation by self-attention mechanism. We use the embedding from RegionDCL~\cite{li2023urban}.
%     \item KnowCL~\cite{liu2023knowledge} integrates knowledge graph and geospatial visual features in inter-view contrastive learning. The knowledge graph is built upon spatial location, type, POIs, and mobility data.
%     \item RegionDCL~\cite{li2023urban} combines building footprints and POIs with a contrastive learning approach by considering building group and regional levels. We feed building footprint, POIs, and AOIs to train the model.
%     \item FactorCL~\cite{factorcl} capture unique and shared information in multiple modalities. We test the extension version of FactorCL by feeding the same three inputs as \modelnamex.
% \end{itemize}

    % \item ReMVC~\cite{tkde} learns intra- and captures mutual information in inter-learning through contrastive learning. We use the same three modalities (POI, AOI, SAT) as inputs, with POI and AOI concatenated before feeding them into the model.

% \begin{itemize}
%     \item Urban2Vec~\cite{wang2020urban2vec}: The original method learns region representations by fusing street view imagery and POI description from Yelp reviews using triplet loss. We retrained the model with satellite imagery and textual data describing POIs and AOIs, including their names and types.
%     \item MVURE~\cite{mvure}: learns region representation by multi-view fusion between POIs and human mobility with graph attention network 
%     combining POIs and human mobility multi-view fusion with graph attention networks  to find regional correlations.
    
%     % by learning a sharing cross-view information between human mobility and urban attributes through multi-view fusion with graph attention networks. We used the embeddings provided by~\cite{li2023urban} using mobility, building footprints, and POIs data. 
%     \item MGFN~\cite{wu2022multi} builds mobility pattern graph and learns regional representation by self-attention mechanism.
%     \item KnowCL~\cite{liu2023knowledge} learns representation by contrastive learning between knowledge graph and geospatial visual feature. The knowledge graph is built upon various data resources, including the spatial location, types, and business categories of POIs and mobility.
%     \item RegionDCL~\cite{li2023urban}: This method learns representations from building footprints and POI data for small partitions first and aggregates into the region level. We extended the method by adding AOI features as the third modality, following the process for encoding POIs. 
%     % jointly learns embedding from building footprints and POIs via contrastive learning at two levels, within building group and with regional level.
% \end{itemize}

% Note that, for a fair comparison, we also run three baselines to take into account the same modalities as \modelname to show the representation performance in the four downstream tasks. The three downstream tasks we run is Urban2Vec [SAT+POI+AOI], MVURE [MOB+BF+POI] and RegionDCL [BF+POI+AOI]. 

% \textbf{Baselines with the same inputs as \modelnamex.} We extend the baseline models with an additional modality to evaluate \modelname using the same input features.
% \begin{itemize}
%     \item Urban2Vec [SAT+POI+AOI]~\cite{wang2020urban2vec}  concatenates AOIs with POIs to match the input features used by \modelnamex.
%     \item MVURE [MOB+BF+POI]~\cite{mvure} incorporates building footprints as an additional modality.
%     \item RegionDCL [BF+POI+AOI]~\cite{li2023urban} combines AOIs and POIs features with the original inputs.
% \end{itemize}





\subsection{Evaluation Metrics}
We evaluate population density, crime rate, and greenness using mean absolute error ($MAE$), root mean square error ($RMSE$), and R-square ($R^2$)~\cite{li2023urban}. 
For the 5-class land use classification (Residential, Industrial, Commercial, Open Space, and Others.), we use L1 distance, KL-divergence, and Cosine similarities~\cite{li2023urban}.

\subsection{Experiment Details}\label{exp:downstream}

\subsubsection{Parameter Settings}
During pretraining, we set the embedding size to 512 for contrastive learning. The final embedding is obtained by concatenating all learned representations from every learning objectives. We use the Adam optimizer for parameter learning with 0.0001 learning rate.

\subsubsection{Downstream Testing Settings}
For regression tasks (population density, crime rate, and greenness), we split the regions  randomly into 5 folds (i.e., 80\% for training and 20\% for testing) and use a random forest regressor for prediction.
% In Table~\ref{table_result_1}, the indication of ($\log	$) represents that the evaluation is performed with a 1-fold train-test split, and the labels were transformed into a logarithmic scale, (i.e., $y = ln(y_{raw} + 1)$)~\cite{liu2023knowledge}. 
For the classification task, we build a hidden dimension of 512 using a 2-layer MLP optimized by KL-divergence loss for 300 epochs~\cite{li2023urban}. 

==> backup/introduction.tex <==
\section{Introduction} 
In the past decade, the global urban population has grown rapidly from 52\% to 57\%~\cite{UNpop}, highlighting the need for effective urban planning and monitoring.
Socioeconomic indicators, such as population density, crime rate, and education level, serve as proxies to understand social and economic dynamics, aiding urban planning decisions that improve quality of life, public health, and community well-being. 
Traditional door-to-door demographic surveys conducted by the US Census Bureau provide detailed statistics but are labor intensive, time consuming, and costly, resulting in infrequent monitoring of cities~\cite{gebru2017using}. 

% you can discuss that there are two main challenges to learn good representations from multi-modal data (you need to mention what can be the modalities,
% Introduce two challenges: intra- and inter-
% Flow: 1) context (background) 2) introduce concepts of RRL and its aim 3) what these rep are used for 4) challenges
The increasing availability of web mapping services, such as OpenStreetMap and Google Maps, has led to an abundance of widely available high-quality geospatial datasets, such as Point-of-Interest (POI) data and satellite/ street view imagery. With these web data, researchers have developed region representation learning to predict various socioeconomic indicators, such as population density, crime rate, or check-ins~\cite{jenkins2019unsupervised, yao2018representing, wang2017region, mvure, liu2023knowledge, li2022predicting}. Their general goal is to learn a region mapping function from web data into vector representations that capture region characteristics by leveraging spatial relationships between regions. 
In general, region representation learning methods tackle the problem following two steps: (1) intra-view learning and (2) inter-view learning. Intra-view learning aims to extract modality-specific features within each modality, and inter-view learning aims to fuse multimodal features within the region.
% (1) extracting region-specific features by considering relationships between regions, and (2) effectively fusing features across multiple data modalities.

% Inclusive, ubiquitous, and frequently updated web data offer high-quality and extensive geospatial datasets globally.  
% With the vast amounts of web data, such as Points-of-Interest (POI) and street view imagery from interactive web mapping services like OpenStreetMap and Google Maps, researchers have developed region representation learning methods, which learn a region mapping function from unlabeled data to vector representations to predict various socioeconomic indicators, such as crime rate, house income, and check-in prediction~\cite{jenkins2019unsupervised, yao2018representing, wang2017region, mvure, liu2023knowledge, li2022predicting}. These approaches typically have two main objectives: intra-view learning, which extracts distinct features within each modality, and inter-view learning, which aims to integrate unique features across modalities.
% evaluate the model's performance by predicting various socioeconomic indicators, such as crime rate, house income, or region check-in prediction~\cite{jenkins2019unsupervised, yao2018representing, wang2017region, mvure}. 
% Recently, many region representation learning models have utilized vast amounts of web data, such as Points-of-Interest (POI) and street view imagery from interactive web mapping services like OpenStreetMap and Google Maps~\cite{liu2023knowledge, li2022predicting, mvure, tkde}. 
% Many region representation learning models often leverage multiple modalities, such as Point-of-Interest (POI), human mobility, and satellite imagery~\cite{liu2023knowledge, li2022predicting, mvure, tkde}. 

% The first challenge is how to extract features considering other regions since the regions are not independent. What are the SOTAs? Graph-based is not okay. Intra-view can do what?
% To address the first challenge, prior works often employ graph-based methods for capturing spatial dependencies by modeling spatial relationships between regions using mobility data or spatial proximity~\cite{zhang2023multi_IJCNN, shin2023understanding, zhou2023heterogeneous}. 
For intra-view learning, prior works often employ graph-based methods for capturing spatial dependencies using mobility data or spatial proximity~\cite{zhang2023multi_IJCNN, shin2023understanding, zhou2023heterogeneous}. 
However, these approaches often rely on predefined region connectivity, such as human mobility or spatial proximity data, limiting their ability to capture region relationships that are not directly captured by the predefined connectivity.
% For example, such as socioeconomic patterns shared by high-income neighborhoods in distant parts of a region.
% To address the first challenge, prior work employs parameterized encoders to learn unique region features from each modality by reconstructing their original input features~\cite{zhang2019unifying}.
% However, these methods assume that regions are independent and identically distributed, overlooking spatial dependencies.
% Graph-based model pros and cons
% To capture these dependencies, graph-based methods have gained popularity by modeling spatial relationships between regions~\cite{jenkins2019unsupervised, mvure, fu2019efficient, zhou2023heterogeneous}. However, these approaches often rely on predefined region connectivity based on mobility data or spatial proximity, limiting their ability to capture region relationships that are not directly captured by the predefined connectivity.

% In intra-view learning, the goal is to capture distinct features within each modality. Traditional methods often use parameterized encoders to reconstruct original features within each view~\cite{zhang2019unifying}. However, these methods assume regions are independent and identically distributed, overlooking spatial dependencies.
% For intra-view learning, the goal is to capture distinct features within each modality by maximizing discrepancies between one and other regions. Traditional methods typically use parameterized encoders to reconstruct the original features within each view~\cite{zhang2019unifying}, but they assume that regions are independent and identically distributed, overlooking spatial dependencies between other regions.
% For intra-view learning, the goal is to ... Traditional methods typically use parameterized encoders to reconstruct the original features within each view~\cite{zhang2019unifying}. However, these reconstruction methods assume that regions are independent and identically distributed, which overlooks spatial dependencies between other regions.

% Graph-based methods have gained popularity for understanding the relationships between regions~\cite{jenkins2019unsupervised, mvure, fu2019efficient, zhou2023heterogeneous}. However, graph-based approaches often rely on heuristic measures, such as predefined region connectivity based on mobility data or spatial proximity. This reliance constrains the model's ability to uncover subtle relationships beyond the initial parameters, which are not directly represented by these heuristics.
% For intra-view learning, the goal is to...
% Traditional methods for feature extraction from each modality typically employ either graph-based techniques~\cite{jenkins2019unsupervised, mvure, fu2019efficient, zhou2023heterogeneous} or learning parameterized encoders by reconstructing original features~\cite{zhang2019unifying}. However, graph-based approaches often rely on heuristic measures, such as predefined region connectivity based on mobility data or spatial proximity. This reliance on predefined parameters can limit the model's ability to discover region relationships beyond these initial parameters, making the model challenging to discover subtle interactions that are not directly captured by the initial heuristics.
% Besides, learning parameterized encoders by reconstructing features may focus on detailed region characteristics. For example, two regions may predominantly contain residential buildings but differ significantly in their land functions due to specific POIs like parks or shops. Such common features may dominate the reconstructed representations, potentially overlooking the distinctive characteristics, which is essential for accurately identifying the regions' functions.

% % Contrastive learning intra-view learning limitation - extra ? 
% But the data is not the technical challenge
% Recent advances in contrastive learning aim to capture distinct region features across modalities by maximizing discrepancies between other regions~\cite{tkde, li2024urban}. However, they often utilize human mobility data as a core modality, which is not widely available everywhere.

% The second challenge is how to effectively fuse features from multiple modalities. The other is since the regions are not independent, how to extract features with the consideration of other regions. What are the SOTA to solve this, ad-hoc methods (concatenation) is not ok, then only shared info (inter-view) is not ok
For inter-view learning, existing methods fuse features from multiple modalities to generate a comprehensive representation that captures diverse geographic characteristics, such as commercial activity represented by shops in POI data and building density observed in satellite imagery. 
A straightforward fusion approach is to combine representations from each view via concatenation~\cite{jenkins2019unsupervised, shin2023understanding, deng2024novel}. However, these methods are ad-hoc and may overlook the inter-modal relationships. In contrast, attention-based fusion methods emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}.
% A straightforward fusion approach is to combine representations from each view via concatenation~\cite{jenkins2019unsupervised, yao2018representing, wang2017region} or weighted averaging with a learnable linear layer to assign importance weights~\cite{mvure}, but these methods are ad-hoc and miss fine-grained, element-wise relationships between modalities. In contrast, attention-based fusion methods emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}.
% through a weighted average~\cite{mvure} with a learnable linear layer assigns importance weights to each modality, but these methods are ad-hoc and fail to capture fine-grained, element-wise relationships between modalities. In contrast, attention-based fusion methods aim to emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}.
% However, these methods are ad-hoc and fail to capture fine-grained, element-wise interactions between modalities, whereas attention-based fusion methods aim to emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}.
% However, these methods are ad-hoc and fail to capture relationships across multiple modalities.
% To overcome these limitations, recent studies use attention-based fusion methods, aiming to emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. 

% To overcome these limitations, recent studies use attention-based fusion methods, aiming to capture various types of correlations across regions and across modalities when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. 
% % However, these methods are ad-hoc and fail to distinguish the most task-relevant features across multiple modalities.  
% % To overcome these limitations, recent studies use attention-based fusion methods, aiming to emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. 

% However, these methods are ad-hoc and fail to distinguish the most task-relevant features within each modality or model the relationships across modalities. 
% For inter-view learning, the goal is to generate a comprehensive representation that captures diverse geographic features across modalities. A straightforward approach combines the representations through concatenation~\cite{jenkins2019unsupervised, yao2018representing, wang2017region} or using a weighted average~\cite{mvure}, where a learnable linear layer assigns importance weights to each modality. 
% % , which employs a learnable linear layer to assign importance weights to each modality before concatenating the learned embeddings. 
% However, these methods are ad-hoc and fail to identify key features within each modality or the relationships across modalities. To overcome these limitations, recent studies use attention-based fusion methods, aiming to emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. 
% these methods often fail to capture complementary information 
However, these methods often fail to align representations across modalities~\cite{tkde, li2024urban}. 
Aligning representations refers to mapping multimodal data into a shared space to make them compatible or comparable.
% Intuitively, multimodal datasets of the same regions tend to be highly correlated within a region and less correlated with other regions. 
% For example, in a commercial area, the POI view may show a high concentration of shops, while the satellite imagery view may reveal a dense distribution of buildings. Together, these modalities reflect the area's commercial activity, complementing each other to provide a comprehensive representation. 
Recent studies propose contrastive learning to align multiple modalities by extracting only shared (mutual) information between modalities~\cite{tkde, li2024urban}. Nevertheless, these approaches may overlook modality-specific (unique) details, which may degrade performance in tasks that rely more on unique features than on shared information~\cite{factorcl, wang2022rethinking}. 
% In order to align multiple modalities that represent the same region, recent studies propose contrastive learning in inter-view learning~\cite{tkde, li2024urban}, which extracts shared (mutual) information between modalities. These approaches predominantly focus on shared information, assuming that the shared information between modalities is almost exactly what is relevant for region representation and the ability to perform various downstream tasks. 
% However, focusing on shared information may overlook task-relevant modal-specific (unique) details and show degraded performance on some downstream tasks when the tasks are less relevant to the shared information and when the downstream tasks are more relevant to the modal-specific information than the shared information~\cite{factorcl, wang2022rethinking}. 

To address this, FactorCL~\cite{factorcl} learns task-relevant unique ($U_{z_1}$, $U_{z_2}$) and shared ($S_{z_{12}}$) information, combining them across two modalities using InfoNCE~\cite{oord2018representation} and CLUB loss~\cite{clubloss}. 
These objectives demonstrate the model's capacity in various domains, such as mortality prediction using tabular health records with sensor data. 
% Specifically, FactorCL achieves $U_{z_1}$, $U_{z_2}$, $S_{z_{12}}$ by maximizing lower bounds of mutual information to capture relevant features while minimizing upper bounds of mutual information to exclude task-irrelevant information, both based on task-related representation $Y$. 
% % Specifically, FactorCL captures task-relevant information and removes task-irrelevant information using InfoNCE and Club loss to capture shared and unique information relevant to the task~\cite{oord2018representation, clubloss}. 
% This objectives demonstrate the model's capacity in various domains, such as mortality prediction using tabular health records with sensor data. 

% Yaoyi's comments on Oct 8th - instead of Table 1, i can address: 
% 1) Cite FactorCL, how their approach achieves better results than using only shared info: first sentence above
% 2) how factorcl works: second & third sentence above
% 3) then continue the complexity (the current paragraph)

% % comments: this is, at the best, an anecdotical statement since no experiment details are given and tested on only limited datasets and tasks. table 2 does not support the statement that 
%  These results indicate the importance of capturing unique information for a comprehensive understanding of region representation
% also, the writing try to explain factorcl in a few sentences but didn't do a good job. for example, all the caluclated by followed by an eq. of I - I + I without explanation is very confusing.

%  instead of your table 1, you should just cite factorcl and say how their approach achive better results than using only shared info. then you briefly talk about how factorcl works and then lead to here and the next paragraph so that it will be clearer what you meant by complexity among modaliries and interaction information term

%  comments: instead of your table 1, you should just cite factorcl and say how their approach achive better results than using only shared info. then you briefly talk about how factorcl works and then lead to here and the next paragraph so that it will be clearer what you meant by complexity among modaliries and interaction information term
%  >> % However, applying FactorCL to more than two modalities becomes computationally expensive because FactorCL requires decomposing shared information across multiple modalities into a combinatorial number of conditional mutual information terms.


% To compare the importance of unique and shared information in region representation learning, Table~\ref{tb:intro} presents the performance of predicting population density and crime rate using POI and Area-of-Interest (AOI) with two FactorCL variants: FactorCL-S, which focuses on task-relevant shared information ($S_{z_{12}}$) by removing task-irrelevant details, and FactorCL-U, which trains on task-relevant unique information by eliminating task-irrelevant shared information ($U_{z_1}$, $U_{z_2}$). 
% % which trains only on the unique information for each modality. 
% Specifically, FactorCL-S captures the shared information between the POI and AOI views regarding as task-relevant representation Y, represented as $S_{\text{POI}\&\text{AOI}}$, and calculated by $I(\text{POI}; \text{AOI}) - I(\text{POI}; \text{AOI}|\text{Y})$. In contrast, FactorCL-U focuses on the unique information for each modality, represented as $U_{POI}$ and $U_{AOI}$, and calculated by $I(\text{POI}; \text{Y}) - I(\text{POI}, \text{AOI}) + I(\text{POI}; \text{AOI}|\text{Y})$.
% As shown in Table~\ref{tb:intro}, FactorCL-U outperforms FactorCL-S, achieving a 5.49\% higher R-squared ($R^2$) for population density prediction and a 3\% increase in $R^2$ for crime rate prediction. These results indicate the importance of capturing unique information for a comprehensive understanding of region representation.

% In Table~\ref{tb:intro}, FactorCL - share is trained by task-relevant shared information and remove task-irrelevant information $I(\text{POI}; \text{AOI})$ - $I(\text{POI};\text{AOI}|\text{Y})$. FactorCL - unique is decomposed into $U_{POI}$ and $U_{AOI}$ and $I(\text{POI}; \text{Y})$ - $I(\text{POI},\text{AOI})$ + $I(\text{POI};\text{AOI}|\text{Y})$, respectively. 
% % In Table~\ref{tb:intro}, FactorCL - share focuses on shared information between POI and AOI, represented as $I(\text{POI}; \text{AOI}; \text{Y})$, while FactorCL - unique incorporates task-specific unique information, $I(\text{POI}; \text{Y} | \text{AOI})$ and $I(\text{AOI}; \text{Y} | \text{POI})$. Specifically, FactorCL - share is expressed as $I(\text{POI}; \text{AOI})$ - $I(\text{POI};\text{AOI}|\text{Y})$, and FactorCL - unique is decomposed into $I(\text{POI}; \text{Y})$ - $I(\text{POI},\text{AOI})$ + $I(\text{POI};\text{AOI}|\text{Y})$ and $I(\text{AOI}; \text{Y})$ - $I(\text{POI},\text{AOI})$ + $I(\text{AOI};\text{POI}|\text{Y})$, respectively.
% As shown in Table~\ref{tb:intro}, FactorCL - unique outperforms FactorCL - share, demonstrating a 5.49\% higher R-squared ($R^2$) for population density prediction and a 3\% improvement in $R^2$ for crime rate prediction. These results indicate the importance of capturing unique information for a comprehensive understanding of region representation.

% Capturing both task-relevant unique and shared information is crucial in region representation learning because the importance of unique and shared information varies by tasks. For example, Table~\ref{tb:intro} presents the performance of predicting population density and crime rate using POI and AOI data with FactorCL variants. 
% FactorCL - share focuses on learning sha`red information from FactorCL, represented as $I(POI; AOI; Y)$, while FactorCL - unique includes task-specific unique information, represented as $I(POI; Y | AOI)$ and $I(AOI; Y | POI)$. 
% FactorCL - share is factorized as $I(POI; AOI) - I(POI;AOI|Y)$, and FactorCL - unique is decomposed into $I(POI; Y) - I(POI,AOI) + I(POI;AOI|Y)$ and $I(AOI; Y) - I(POI,AOI) + I(AOI;POI|Y)$, respectively. 
% As shown in Table~\ref{tb:intro}, FactorCL - unique demonstrates 5.49\% higher R-squared ($R^2$) than FactorCL - share in predicting population density. Similarly, FactorCL - unique shows a 3\% improvement in $R^2$ compared to FactorCL - share in crime rate prediction. These results indicate the importance of capturing unique information for a comprehensive understanding of region representation.
% Thus, recent studies propose contrastive learning to align representations by maximizing shared (mutual) information across modalities, ensuring information consistency in the combined representation~\cite{tkde, li2024urban}. 
% However, by focusing predominantly on shared information, contrastive learning may overlook modality-specific details that could be important for certain downstream tasks~\cite{wang2022rethinking}.
% Intuitively, not only sharing the information, but also preserving unique information, is crucial in region representation learning because some tasks are possibly more relevant to a specific modality than other modalities.
% For instance, Table~\ref{tb:single_modal} shows that Area-of-Interest (AOI) is more predictive of population and crime than others, such as Point-of-Interest (POI), indicating task relevance varies across modalities.  

% To address this, FactorCL~\cite{factorcl} in multi-modal learning preserves both task-relevant unique and shared information while fusing two modalities, demonstrating effectiveness in various domains, such as mortality prediction using tabular health records with sensor data. 

%  factorcl (unique) vs (shared) vs (u+s) 
% \begin{table}[htbp]
% \centering
% \caption{$R^2$ of predicting NYC population density and crime rate using FactorCL variants with POI and AOI}
% \begin{adjustbox}{width=0.6\columnwidth,center}
%   \begin{tabular}{l | c | c  }  \toprule
%   Methods  & Population & Crime\\ \midrule
%   FactorCL-S & 0.384 & 0.175 \\
%   FactorCL-U & 0.439 & 0.205 \\
%   % FactorCL & 0.547 & 0.279 \\ 
%   \bottomrule
%   \end{tabular}
%   \label{tb:intro}
% \end{adjustbox}
% \end{table}

%  FactorCL applying to multiple modalities are computationally expensive
%  With factorcl, calculating I(x_i; x_j; x_k; Y | x_l) is complex since it involves a number of factorizations (e.g., in 4 modalities, 16). So itis complex. 
However, applying FactorCL to more than two modalities becomes computationally expensive because FactorCL requires decomposing shared information across multiple modalities into a combinatorial number of conditional mutual information terms.
% FactorCL requires factorizing shared information across multiple InfoNCE and CLUB losses, which estimate mutual information by calculating conditional probabilities between modality pairs.
% utilize an interaction information term, which decomposes shared information among multiple modalities into mutual information components. 
% the complexity among modalities by using an interaction information term, which decomposes shared information among multiple modalities into mutual information components.
Specifically, there are $2^M-1$ possible combinations representing distinct shared and unique information with $M$ modalities. For example, with three modalities ($m_1$, $m_2$, $m_3$), the task-relevant objectives are individual, pairwise, and triplet sets ($U_{z_1}$, $U_{z_2}$, $U_{z_3}$, $S_{z_{12}}$, $S_{z_{13}}$, $S_{z_{23}}$, $S_{z_{123}}$), a total of 7. For four modalities, this expands to $15$ combinations.
% (1, 2, 3, 12, 13, 23, 123), 
Excluding unique information, a total of $2^M-1-M$ distinct shared information objectives remain, each of which is again decomposed into multiple conditional mutual information terms, leading to prohibitive complexity.

% each requiring multiple InfoNCE and CLUB loss terms for optimization. 
% applying FactorCL to more than two modalities becomes computationally expensive due to the need to factorize shared information across several InfoNCE and CLUB losses~\cite{factorcl}. 
% These losses are expensive because InfoNCE, commonly used in contrastive learning, requires the comparison of many positive and negative sample pairs, increasing the computational complexity as the number of modalities grows. Similarly, CLUB loss estimates mutual information by calculating the conditional probability between modality pairs.  
% Specifically, FactorCL decomposes shared information using an interaction information term, which decomposes shared information among multiple modaltiies into mutual information form, and eliminates duplicate learning objectives.
% With $M$ modalities, there are $2^M-1$ possible combinations representing distinct shared and unique information. Excluding unique information, a total of $2^M-1-M$ distinct shared information objectives remain, each requiring multiple InfoNCE and CLUB loss terms for optimization.  
% However, applying FactorCL to more than two modalities increases computational complexity because the number of learning objectives grows exponentially. 
% For instance, with four modalities ($x_i$, $x_j$, $x_k$, $x_l$), calculating the task-relevant shared information $I(x_i; x_j; x_k; Y | x_l)$ involves a complex interaction information process (i.e., a generalization of the mutual information for more than two variables), extending mutual information to multiple variables until mutual information form like $I(x_1;x_2)$. 
% Additionally, $Y$ represents the concatenation of all augmentation pairs in self-supervised learning~\cite{sordoni2021decomposed}, resulting in high-dimensional computations. As the number of modalities grows, optimization becomes increasingly challenging due to the rising dimensionality and computational complexity.

% Pairwise intuition
% intuition is lacking. this part we dont need, and we lose. but it is okay. we will show that
% show what do we lose, why do we think it is not necessary in pair wise
% To reduce the complexity, one of the solutions is to focus on pairwise interactions between modalities, which are often sufficient for capturing task-relevant, modal-specific information. 
Although FactorCL captures the shared information among more than two modalities using conditional mutual information, such as triplet (e.g., $S_{z_{123}}$) or quadratic interaction (e.g., $S_{z_{1234}}$) among four modalities, pairwise interactions (e.g., $S_{z_{12}}$) are often satisfactory~\cite{musciotto2021detecting} to capture key patterns without requiring additional shared information among three or more modalities, i.e., high-order combinations.
While high-order combinations can capture additional details, the core insights are often adequately captured through the interactions between pairs of modalities.
For example, if satellite imagery and AOI already identify an area as a park (e.g., leisure area), adding POI that indicates a playground or trail does not provide new information but only confirms what is already known.

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/intro_.png}
    \caption{Modality-specific information and shared information in pairwise interaction among three input modalities}
    \label{intro_fig}
\end{figure}

% Although unique and shared information between every possible information is important, pairwise interactions are sufficient to capture important patterns without the need for high-order combinations~\cite{musciotto2021detecting} in region representation learning.
% In region representation learning, pairwise interactions are sufficient to capture task-relevant, modal-specific information without requiring higher-order combinations, which involve interactions among more than two modalities. 
% Introducing higher-order combinations, such as using satellite imagery, POI, and AOI together, may capture additional details; however, the core insights are often already reflected in the interaction between pairs of modalities.
% While high-order combinations, such as integrating satellite imagery, POI, and AOI, can capture additional details, the core insights are often adequately captured through the interactions between pairs of modalities by pairwise perspective.
% For example, the interaction between satellite imagery and POI can reveal land use patterns, distinguishing between commercial and residential areas based on building distribution and human activities.
% % Introducing higher-order combinations, such as using satellite imagery, POI, and AOI together, may capture additional details; however, the core insights are often already reflected by the interaction between pairs of modalities.
% % Introducing higher-order combinations, such as using satellite imagery, POI, and AOI together, may capture some additional details but often results in redundancy. 
% In particular, if satellite imagery and AOI already identify an area as a park (e.g., leisure area), adding POI that indicates a playground or trail does not provide new information but only confirms what is already known. 

We propose a pairwise inter-view learning approach that considers all modalities in pairs, focusing on each pair's shared information while preserving distinctive features learned through intra-view learning. 
Figure~\ref{intro_fig} shows the task-relevant modality-specific feature and shared feature in pairwise approach in inter-view learning. Particularly, the pairwise inter-view learning optimizes both $U_{z_S}$ and $S_{z_{SA}}$ for all possible pairs while neglecting shared information associated with more than three modalities.
Built on this pairwise inter-view learning, we propose a multimodal region representation approach, \modelname \footnote{\modelname refers to \textbf{C}r\textbf{O}ss m\textbf{O}dal \textbf{K}nowledge \textbf{I}njected \textbf{E}mbedding}\logov with two primary goals: capturing (1) region features within each modality via intra-view learning, and (2) task-relevant modality-specific and shared information through pairwise inter-view learning. 
% \modelname has two primary goals: (1) intra-view learning within each modality, and (2) pairwise inter-view learning between modalities.
Figure~\ref{cookie_method} illustrate \modelnamex's overall approach. It first pretrains each modality encoder by maximizing region discrepancies to capture region features. Then, 

Figure 2 shows CooKIE’s approach: it first pretrains each modality encoder by maximizing regional discrepancies through intra-view learning, then captures task-relevant unique and shared information with pairwise inter-view learning to blend modalities effectively."

% In intra-view learning, \modelname extracts region representations by maximizing the discrepancy between regions using contrastive learning. 
% In pairwise inter-view learning, \modelname captures task-relevant shared and unique information between modalities, improving the complexity over high-order combinations by efficiently capturing key insights without the computational burden of high-order interactions.
To demonstrate \modelnamex, we input POI, AOI, satellite imagery, and building footprint to generate the learned region vector and evaluate the representation using several downstream tasks, such as population density, crime rate, land use classification, and greenness score prediction.
% by inputting POI, AOI, satellite imagery, and building footprint and outputting the learned region vector representing for each region. 

% where pairwise interactions are sufficient to capture key patterns without high-order combinations.
% In pairwise inter-view learning, \modelname aims to learn task-relevant shared information and maintain unique information by optimizing mutual information bounds.
% In pairwise inter-view learning, \modelname aims to learn task-relevant shared information and maintain unique information by maximizing mutual information lower bounds while minimizing task-irrelevant information using mutual information upper bounds.

The contributions of our paper are as follows,
\begin{itemize}
    \item We propose a region representation learning framework, \modelnamex, to learn region vectors from an arbitrary number of modalities obtained from web mapping services.
    \item \modelname captures both task-relevant shared and modality-specific information. We evaluate \modelname by predicting several downstream tasks such as population density, crime rate, land use classification, and greenness predictions in NYC and Delhi, where geospatial data distributions vary.
    \item \modelname demonstrates low computational complexity by reducing to O($n^2$) complexity.
    % \item We propose a pairwise inter-view fusion to capture task-relevant shared information and preserve modal-specific features in region representation learning by mutual information bounds.
    % \item We simplify an extension of FactorCL to reduce the computational complexity for more than two modalities and demonstrate the effectiveness by evaluating our model's ability in New York City (NYC) and Delhi, where geospatial data distributions vary.
\end{itemize}

% % concat
% With the proliferation of geospatial data, researchers have developed region representation learning methods, which learn a region mapping function from unlabeled data to vector representations to predict socioeconomic indicators using multiple data sources~\cite{jenkins2019unsupervised, yao2018representing, wang2017region}. These methods use ad-hoc methods to fuse features, such as concatenation or weighted sum, which expects machine learning models to select and combine these features effectively. However, without explicitly considering the inter-relationships between modalities and between regions might overlook inter-modality correlation. 
% % However, these methods fuse representations from multiple modalities using concatenation or weighted sum techniques, overlooking inter-modality correlations.

% multi-view: intra-view learning
% Further, recent studies have focused on fusing multiple modalities to capture the multidimensional characteristics of regions~\cite{mvure, luo2022urban, zhou2023heterogeneous}. Typically, multi-modal fusion involves two main pipelines: (1) intra-view learning, which extracts modality-specific features within each region, and (2) inter-view learning, which fuses these features into a comprehensive region representation. 
% In particular, traditional intra-view learning methods, such as graph-based techniques~\cite{jenkins2019unsupervised, mvure, fu2019efficient} or feature reconstruction~\cite{zhang2019unifying}, often rely on heuristic measures or focus on detailed features that may not effectively differentiate regions~\cite{tkde}. 
% To address this, recent approaches~\cite{tkde, li2024urban} use contrastive learning in intra-view learning to maximize discrepancies between regions, showing promising results. 

% multi-view: inter-view learning ; attention and contrastive lr
% In multi-view fusion, one type of approaches use attention mechanisms to combine representations from modalities~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. 
% Although these methods extract key features from each modality, they often fail to align shared information across modalities~\cite{li2024urban}. 
% In region representation learning, it is essential that information from multiple views is highly correlated for the same region and less correlated for other regions. For example, a region may be identified as a commercial area if a Point-of-interest (POI) contains shops and satellite imagery indicates a dense distribution of buildings typical of a business district.
% Therefore, \citet{tkde} and \citet{li2024urban} propose contrastive learning between views by serving as constraints to each other within the same region and enforcing information to be consistent across views.
% However, since this approach heavily focuses on the shared information, potentially overlooking modality-specific details important for downstream tasks~\cite{wang2022rethinking}.

% To tackle this challenge, FactorCL~\cite{factorcl} preserves both unique and shared information while fusing two modalities, demonstrating effectiveness in various domains, such as mortality prediction using tabular health records with sensor data. Intuitively, not only the shared information but also preserving unique information is crucial in region representation learning because some tasks are possibly more relevant to a specific modality than other modalities.
% For instance, Table~\ref{tb:single_modal} shows that Area-of-Interest (AOI) is more predictive of population and crime than others, such as Point-of-Interest (POI), indicating task relevance varies across modalities. 
% Therefore, preserving unique information for each modality is necessary to generate a comprehensive region representation.


% However, applying FactorCL to more than two modalities introduces high computational complexity. Specifically, increasing the number of modalities exponentially increases the number of learning objective terms (i.e., loss functions). 
% % For instance, assuming there are four modalities ($x_i$, $x_j$, $x_k$, $x_l$), the task-relevant shared information between $x_i$, $x_j$, $x_k$ is $\arg\max_{}I(x_i;x_j;x_k;Y|x_l)$, which maximizes the shared information among $x_i$, $x_j$, $x_k$, and task-relevant semantic $Y$ conditioned on $x_l$, 
% For instance, assuming there are four modalities ($x_i$, $x_j$, $x_k$, $x_l$), the task-relevant shared information between $x_i$, $x_j$, $x_k$ and $Y$ can be expressed as $I(x_i; x_j; x_k; Y | x_l)$. In self-supervised learning, $Y$ can be proxies of a combination of all augmentation pair of $x_i; x_j; x_k$. 
% Specifically, estimating shared information among four modalities requires further decomposition using interaction information to formulate the mutual information term.
% Therefore, as the number of objectives increases, computing each mutual information loss function becomes challenging due to the curse of dimensionality. 

% To address the aforementioned challenges, we propose a multi-modal region representation learning approach, \modelnamex\footnote{\modelname refers to \textbf{C}r\textbf{O}ss m\textbf{O}dal \textbf{K}nowledge \textbf{I}njected \textbf{E}mbedding}\logo, which consists of intra-view learning and inter-view learning. 
% Inspired by the recent success using contrastive learning in intra-view learning~\cite{tkde, li2024urban}, we aim to learn unique view-specific information by discriminating with other regions for each view through intra-view learning. 
% We then simultaneously preserve the unique information and extract the shared information from multiple modalities ($N \geq 3$) using a pairwise inter-view fusion approach. Our proposed approach constructs all possible pairwise modalities to extract unique and shared information, diminishing the number of learning objectives and reducing the complicated interaction information. 
% Inspired by Imagebind~\cite{imagebind}, which employs the image as a central representation to connect other modalities, we propose that the region itself serves as the binding representation in our context. Intuitively, all geospatial data associated with the same region inherently ties together, ensuring consistency across multiple pairs. 

% The contributions of our paper are as follows,
% \begin{itemize}
%     \item We propose pairwise inter-view fusion to capture shared and preserve unique information to learn informative and consistent region representations across multiple modalities. This approach maximizes shared information while minimizing task-irrelevant information from a pairwise perspective in multi-modal region representation learning.
%     \item We simplify an extension version of FactorCL to reduce the computational complexity when more than two modalities exist and demonstrate the effectiveness by evaluating its' ability in New York City (NYC) and Delhi, where the distribution of geospatial data varies. 
% \end{itemize}
% \modelname aims to simultaneously capture the unique and shared information from multiple modalities ($N \geq 3$) using a pairwise fusion approach. 
% Our proposed fusion approach constructs possible pairwise to extract unique and consistent information, diminishing the number of optimization goals and reducing the complicated conditional information compared to merely extending FactorCL across three modalities.  
% Inspired by Imagebind~\cite{imagebind}, which employs the image as a central element to connect other modalities, we propose that the region itself serves as the binding representation in our context. Intuitively, all geospatial data associated with the same region inherently ties the modalities together, ensuring consistency and relevance across multiple pairs. 
% We further incorporate intra-view learning, which extracts unique region information from each modality to enhance the pairwise fusion approach, as inspired by~\cite{tkde, li2024urban, mvure}. 

% leave the end


% These methods are typically built upon graph-based or utilize data that contains region relationships such as human mobility and spatial proximity, which is limited to the models' applicability.
% These methods typically build graph structure~\cite{wu2022multi_mgfn, mvure, wang2017region} or contrastive learning~\cite{tkde, li2024urban} using human mobility or spatial proximity to represent relationships between regions. However, almost all existing models still require a feature vector for each region to discover region correlation. 

% the feature vector must integrate multiple perspectives of regions, since socioeconomic indicators reflect the diverse and complex nature of regions.
% To address this, recent studies fuse multiple modalities to incorporate the multifaceted perspective in inter-view learning using attention mechanisms~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. Although these methods extract significant features from each modality, attention-based methods often fail to align shared information between modalities~\cite{tkde, li2024urban}, which is a crucial perspective that lies in region representation learning. Specifically, each modality that represents the same region is often correlated. Thus, the representation for each modality should be consistent. 

% Contrastive learning methods~\cite{tkde, li2024urban} aim to align representations between modalities by capturing consistent information. However, focusing primarily on shared information can overlook modality-specific details. This is because modality-specific unique information might be more relevant than consistent information, and the importance of unique information for each modality is varied across certain tasks~\cite{factorcl}. 
% To tackle this challenge, FactorCL~\cite{factorcl} preserves both unique and shared information while fusing two modalities, demonstrating its effectiveness in various domains, such as mortality prediction using health records or sentiment analysis using videos. Intuitively, not only the shared information but also preserving unique information is crucial in region representation learning because some tasks are possibly more relevant to a specific modality than others.
% For example, Area-of-Interest (AOI) is more predictive of population and crime than other modalities such as Point-of-Interest (POI), while satellite imagery performs better than others in greenness, shown in Table~\ref{tb:single_modal}). Therefore, preserving unique information for each modality is necessary to generate a comprehensive representation for region representation learning.

% However, extending FactorCL to more than two modalities introduces high complexity due to higher dimensionality and more intricate optimization goals, which leads to complicated and elongated feature vectors. 
% Additionally, optimizing mutual information among multiple modalities becomes increasingly challenging, as it involves high-dimensional conditions. 
% For example, assuming there are three modalities ($Z_i$, $Z_j$, $Z_k$), the task-relevant mutual information between $Z_i$ and $Z_j$ is $\arg\max_{}I(Z_i;Z_j;Y|Z_k)$, which maximizes mutual information among $Z_i$, $Z_j$, and $Y$ conditioned on $Z_k$. Factoring this term requires considering $Z_k$, and additional conditional information (i.e., interaction information), which can lead to ad-hoc and abstract formulations. 

% \begin{figure}
% \vspace{-0.8em}
% \setlength{\belowcaptionskip}{-9pt}
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/t1.png}
%         \caption{Single modal testing}
%         \vspace{2em}
%         % \vspace{-2em}
%         \label{all_single}
%     \end{subfigure}
%     \vspace{3em}
%     \hfill
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/t1.png}
%         \caption{Multi modal testing}
%         \label{all_multi}
%         \vspace{-1em}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/t1.png}
%         \caption{Multi modal testing}
%         \label{all_multi}
%         % \vspace{-2em}
%     \end{subfigure}
%     \vspace{2em}
%     \caption{Modality Performance Testing}
%     \label{all_testing}
%     \hfill
% \end{figure}

% % leave the end
% The contributions of this paper are as follows,
% \begin{itemize}
%     \item We propose pair-wise fusion in region representation learning, called \modelnamex, which captures shared and preserves unique features for each modality. To the best of our knowledge, \modelname is the first method to capture the shared and preserve unique information in RE
%     % We propose a generalized multi-modal region representation learning method, \modelnamex, aiming to learn task-relevant view-specific and shared information by incorporating more than two modalities.
%     % To the best of our knowledge, this is the first work to optimize both mutual and unique features in more than two input modalities in the region representation learning. 
%     \item We simplify an extension version of FactorCL to reduce the complexity when more than two modalities exist and demonstrate the effectiveness by evaluating its' ability in New York City (NYC) and Delhi, where the distribution of geospatial data varies. 
%     % regions where much geospatial data is not available (Delhi, India). 
%     % \item \modelname demonstrates generalizability in multi-modal learning when more than two modalities are available in region representation learning.
%     % \item We demonstrate \modelnamex's ability in Delhi (India), especially for the region where much geospatial data is not available. 
%     % \item \modelname shows the state-of-the-art performance in greenness downstream task, which is directly related to human health on a daily basis. This highlights \modelnamex's potential for bridging regional representation learning and public health analysis.
% \end{itemize}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/MI.png}
%     \vspace{0.5em}
%     \caption{Multi-modal Information Diagram}
%     \label{mi_fig}
% \end{figure}


==> backup/introduction__1_.tex <==
\section{Introduction} 
In the past decade, the global urban population has grown rapidly from 52\% to 57\%~\cite{UNpop}, highlighting the need for effective urban planning and monitoring.
Socioeconomic indicators, such as population density, crime rate, and education level, serve as proxies to understand social and economic dynamics, aiding urban planning decisions that improve quality of life, public health, and community well-being. 
Traditional door-to-door demographic surveys conducted by the US Census Bureau provide detailed statistics but are labor intensive, time consuming, and costly, resulting in infrequent monitoring of cities~\cite{gebru2017using}. 

% RRL goal, intuition intra and inter, define terms
With the increasing availability of geospatial data online, researchers have used these data obtained from web, such as Point-of-Interest (POI) data, satellite imagery, and street view imagery, to study the region representation learning problems~\cite{jenkins2019unsupervised, yao2018representing, wang2017region, mvure, liu2023knowledge, li2022predicting}. 
Their goal is to learn a region mapping function from multiple modalities into a representation space that captures region characteristics, such as relationships between regions and interactions between modalities. 

% comments: such as region rel & modal rel 
% region rel -> 1) graph, 2) intra view ( region negative...)
% modal rel -> 1) concat; type of modal rel, 2) inter-view

%  these two defs are not necessary... 
% Learning a representation for each modality, namely intra-view learning, allows the models to reflect the attributes specific to each data source, thereby fully expressing the information that each modality contains.
% Learning a representation within each modality, namely intra-view learning, allows the models to reflect the attributes specific to each modality. 
% Additionally, capturing interactions between modalities, known as inter-view learning, enables the models to combine complementary features, which generates a comprehensive region representation.
% The increasing availability of web mapping services, such as OpenStreetMap and Google Maps, has led to an abundance of widely available high-quality geospatial datasets, such as Point-of-Interest (POI) data and satellite and street view imagery. With these web data, researchers have studied the region representation learning problem to predict various socioeconomic indicators, such as population density, crime rate, and check-ins~\cite{jenkins2019unsupervised, yao2018representing, wang2017region, mvure, liu2023knowledge, li2022predicting}. Their general goal is to learn a region mapping function from web data into a representation space that captures region characteristics, such as the spatial relationships between regions and .... 
% These methods tackle the problem in two steps: (1) intra-view learning and (2) inter-view learning. Intra-view learning aims to extract representations within each modality, and inter-view learning further aims to fuse multimodal features within the region.


% First, \modelname aims to learn the region representations of a modality that are distinctive across regions using intra-view learning. Secondly, we propose a pairwise inter-view learning method to further optimize the representations by capturing task-relevant shared information between pairs of modalities and modality-specific information.
To learn relationships between regions, previous works use graph-based methods to capture spatial dependencies using predefined region connectivity, such as mobility data or spatial proximity defined by edges~\cite{zhang2023multi_IJCNN, shin2023understanding, zhou2023heterogeneous}. 
However, these approaches often rely on predefined connectivity, limiting their ability to capture region relationships that are not directly captured by the predefined connectivity. In other words, they may overlook indirect influences between regions that extend beyond the predefined connectivity, which fails to address comprehensive region relationships. To address this, recent studies leverage contrastive learning~\cite{chen2024rrl_survey, tkde, li2024urban} that maximizes discrepancies between regions. 
These methods can capture a representation for each modality by comparing other regions, demonstrating their superiority in region representation learning compared to other approaches.

% For intra-view learning, earlier approaches utilize autoencoders to capture a representation for each modality by reconstructing the original input features~\cite{zhang2019unifying}. However, this approach may overemphasize dominant features, leading to similar representations for distinct regions~\cite{tkde}. 
% For instance, two regions share prevalent residential POIs, yet differ in land function due to unique attributes such as parks or bars. 
% In this case, the residential POIs might dominate the learning process, which results in similar representations for both regions.
% To address this, recent studies leverage contrastive learning~\cite{chen2024rrl_survey, tkde, li2024urban} that maximizes discrepancies between regions. 
% These methods can capture a representation for each modality by comparing other regions, demonstrating their superiority in region representation learning compared to other approaches.
% Building on this success, we propose learning representations from each modality through comparisons with other regions, which can capture and distinguish the unique attributes of each region. 

% To learn spatial relationships between regions, previous work use graph-based methods to capture spatial dependencies using predefined region connectivity, such as mobility data or spatial proximity defined by edges~\cite{zhang2023multi_IJCNN, shin2023understanding, zhou2023heterogeneous}. 
% However, these approaches often rely on predefined connectivity, limiting their ability to capture region relationships that are not directly captured by the predefined connectivity. In other words, they may overlook indirect influences between regions that extend beyond the predefined connectivity, which fails to address comprehensive region relationships. 
% To address the first challenge, prior work employs parameterized encoders to learn unique region features from each modality by reconstructing their original input features~\cite{zhang2019unifying}.
% However, these methods assume that regions are independent and identically distributed, overlooking spatial dependencies.

% Graph-based methods have gained popularity for understanding the relationships between regions~\cite{jenkins2019unsupervised, mvure, fu2019efficient, zhou2023heterogeneous}. However, graph-based approaches often rely on heuristic measures, such as predefined region connectivity based on mobility data or spatial proximity. This reliance constrains the model's ability to uncover subtle relationships beyond the initial parameters, which are not directly represented by these heuristics.
% For intra-view learning, the goal is to...
% Traditional methods for feature extraction from each modality typically employ either graph-based techniques~\cite{jenkins2019unsupervised, mvure, fu2019efficient, zhou2023heterogeneous} or learning parameterized encoders by reconstructing original features~\cite{zhang2019unifying}. However, graph-based approaches often rely on heuristic measures, such as predefined region connectivity based on mobility data or spatial proximity. This reliance on predefined parameters can limit the model's ability to discover region relationships beyond these initial parameters, making the model challenging to discover subtle interactions that are not directly captured by the initial heuristics.
% Besides, learning parameterized encoders by reconstructing features may focus on detailed region characteristics. For example, two regions may predominantly contain residential buildings but differ significantly in their land functions due to specific POIs like parks or shops. Such common features may dominate the reconstructed representations, potentially overlooking the distinctive characteristics, which is essential for accurately identifying the regions' functions.

% For modality rel, ... concat... but.. inter
For inter-view learning, existing methods fuse features from multiple modalities to generate a comprehensive region representation that reflects diverse geographic characteristics, like commercial activity from POI data and building density from satellite imagery. A straightforward approach is to concatenate the representations of each modality for predictions~\cite{jenkins2019unsupervised, shin2023understanding, deng2024novel}. However, these methods are ad-hoc and may overlook the interactions between modalities. To overcome this, researchers study attention-based techniques that emphasize important features from each modality during integration~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. 

% For inter-view learning, existing methods fuse features from multiple modalities to generate a comprehensive region representation that reflects diverse geographic characteristics, such as commercial activity represented by shops in POI data and building density observed in satellite imagery. 
% A straightforward approach is to concatenate the representations from each modality for prediction~\cite{jenkins2019unsupervised, shin2023understanding, deng2024novel}. However, these methods are ad-hoc and may overlook the interactions between modalities. 
% To address the limitation of the lack of interaction, researchers study attention-based methods that emphasize important features from each modality when integrating representations~\cite{zhou2023heterogeneous, sun2024urban, wu2022multi_mgfn}. Although attention mechanisms account for interactions between modalities by focusing on key features, they often fail to align representations across modalities~\cite{tkde, li2024urban}. Aligning representations refers to mapping multimodal data into a shared space to ensure compatible or comparable.

Although attention mechanisms enhance interactions by focusing on key features, they often fail to align representations across modalities~\cite{tkde, li2024urban}. Aligning representations refers to mapping multimodal data into a shared space, ensuring compatibility and comparability.
Recent studies use contrastive learning to align modalities by capturing shared (mutual) information between modalities~\cite{tkde, li2024urban}. Yet, these approaches may overlook modality-specific (unique) details, which can be important to the prediction tasks~\cite{factorcl, wang2022rethinking}.
% which may degrade performance in prediction tasks that rely more on unique features than on shared information~\cite{factorcl, wang2022rethinking}. 
Expanding beyond region representation learning, FactorCL~\cite{factorcl} address the challenge by capturing both task-relevant unique ($U_{z_1}$, $U_{z_2}$) and shared ($S_{z_{12}}$) information between two modalities using InfoNCE~\cite{oord2018representation} and CLUB loss~\cite{clubloss}. 
This method shows promising results in various domains, such as mortality prediction using tabular health records with sensor data. 

However, applying FactorCL to more than two modalities becomes computationally expensive because FactorCL requires decomposing shared information across multiple modalities into a combinatorial number of conditional mutual information terms.
Specifically, with $M$ modalities, there are $2^M-1$ possible combinations representing distinct shared and unique information. For instance, with three modalities ($d_1$, $d_2$, $d_3$), the objectives include the computation of individual, pairwise, and triplet sets ($U_{z_1}$, $U_{z_2}$, $U_{z_3}$, $S_{z_{12}}$, $S_{z_{13}}$, $S_{z_{23}}$, $S_{z_{123}}$), a total of 7. With four modalities, the number of combinations increases to $15$ combinations. 
Therefore, decomposing information in FactorCL is prohibitively complex as the number of modalities grows.
% Excluding unique information, a total of $2^M-1-M$ distinct shared information objectives remain, each of which is again decomposed into multiple conditional mutual information terms, leading to prohibitive complexity.
% refer to prev works (citation) : how they argue pairwise nodes are enough? 
Although FactorCL captures shared information among more than two modalities like triplets (e.g., $S_{z_{123}}$) or quadruplets (e.g., $S_{z_{1234}}$), focusing on pairwise interactions (e.g., $S_{z_{12}}$) often suffices to capture key patterns.
This approach can effectively reflect essential relationships without needing additional shared information among three or more modalities, i.e., high-order combinations. 
While high-order combinations can provide additional details, the core insights are adequately captured through the interactions between pairs of modalities.
For example, if satellite imagery and AOI data already identify an area as a park (e.g., leisure area), adding POI data that indicates a playground or trail does not provide new information but only confirms what is already known.

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/intro_.png}
    \caption{Modality-specific information and shared information in pairwise interaction among three input modalities and task-relevant semantics $z^\prime$}
    \label{intro_fig}
\end{figure}

% Although unique and shared information between every possible information is important, pairwise interactions are sufficient to capture important patterns without the need for high-order combinations~\cite{musciotto2021detecting} in region representation learning.
% While high-order combinations, such as integrating satellite imagery, POI, and AOI, can capture additional details, the core insights are often adequately captured through the interactions between pairs of modalities by pairwise perspective.
% In particular, if satellite imagery and AOI already identify an area as a park (e.g., leisure area), adding POI that indicates a playground or trail does not provide new information but only confirms what is already known. 


Therefore, we propose a pairwise inter-view learning method that considers all modalities in pairs, focusing on each pair's shared information to achieve comprehensiveness and computational efficiency when fusing more than two modalities.
Figure~\ref{intro_fig} illustrates how pairwise inter-view learning captures task-relevant modality-specific and shared features.
Specifically, $U_{z_S}$ represents the mutual information between the $S$ modality and task-relevant semantics $z^\prime$ conditioned on other input modalities. Similarly, $S_{z_{SA}}$ denotes the shared information among $S$, $A$ modality, and $z^\prime$ conditioned on the other remaining input modality. 

Building on this pairwise inter-view learning, we propose a multimodal region representation approach, \modelname \footnote{\modelname refers to \textbf{C}r\textbf{O}ss m\textbf{O}dal \textbf{K}nowledge \textbf{I}njected \textbf{E}mbedding}\logov with two primary goals.
First, we aim to capture region-specific attributes for each modality through intra-view learning, allowing \modelname to fully express the characteristics of each data modality. 
Second, we leverage pairwise inter-view learning to capture task-relevant information that spans both modality-specific and shared features across modalities.
Specifically, for intra-view learning, we utilize contrastive learning to generate representations for each modality by comparing regions within the same modality, inspired by~\cite{tkde, li2024urban}. 
We then integrate these representations using pairwise inter-view learning, which accounts for both individual modality attributes and shared information between pairs.
To demonstrate \modelnamex, we use POI, AOI, satellite imagery, and building footprint to learn region vectors and evaluate the representations using several downstream tasks, such as population density, crime rate, greenness score prediction, and land use classification.

% In intra-view learning, we compare each region with other regions to learn each modality's representation through contrastive learning, inspired by~\cite{tkde, li2024urban}. Then, we fuse the learned representation from each modality by considering both modality-specific and shared information via pairwise inter-view learning. 

% Figure~\ref{cookie_method} illustrates \modelnamex's overall approach. \modelname first pretrains each modality encoder to capture representations by maximizing the discrepancy between regions using contrastive learning. Then, \modelname learns both modality-specific and shared information through pairwise inter-view learning. Finally, \modelname jointly optimizes intra- and pairwise inter-view learning across all modality pairs together.
% In intra-view learning, \modelname extracts region representations by maximizing the discrepancy between regions using contrastive learning. 
% In pairwise inter-view learning, \modelname captures task-relevant shared and unique information between modalities, improving the complexity over high-order combinations by efficiently capturing key insights without the computational burden of high-order interactions.
% by inputting POI, AOI, satellite imagery, and building footprint and outputting the learned region vector representing for each region. 

The contributions of our paper are as follows,
\begin{itemize}
    \item We propose a region representation learning approach, \modelnamex, to learn region embeddings from an arbitrary number of modalities obtained from web.
    \item \modelname captures both task-relevant shared and modality-specific information. We evaluate \modelname by predicting several downstream tasks such as population density, crime rate, land use function, and greenness in NYC and Delhi, where geospatial data distributions vary.
    \item We demonstrate that \modelname has a lower computational complexity compared to existing methods,  reducing the complexity from O($2^m$) to O($m^2$) with $m$ modalities.
    % \item We propose a pairwise inter-view fusion to capture task-relevant shared information and preserve modal-specific features in region representation learning by mutual information bounds.
    % \item We simplify an extension of FactorCL to reduce the computational complexity for more than two modalities and demonstrate the effectiveness by evaluating our model's ability in New York City (NYC) and Delhi, where geospatial data distributions vary.
\end{itemize}


==> backup/methodology.tex <==
\section{\modelnamex}
Figure~\ref{cookie_method} illustrates the overall approach of \modelnamex. 
\modelname first pretrains an encoder for each modality to extract the representative features of each region within each modality by a contrastive learning approach. 
Then, \modelname learns task-relevant modality-specific and shared information through pairwise inter-view learning to effectively blend representations from multimodal data. 

%     \caption{\modelname consists of two objectives. (a) intra-view learning aims to learn unique region features within each modality by comparing with other regions. (b) pairwise inter-view learning aims to learn task-relevant unique and shared information.}

\begin{figure}[h]
    \centering
\includegraphics[width=0.45\textwidth]{figures/icdm-aaai-fig-v2.png}
    \vspace{0.5em}
    % \caption{\modelname consists of intra-view learning and pairwise inter-view learning.}
    \caption{\modelname consists of two parts: (a) intra-view learning, which captures representations within each modality by comparing with other regions, and (b) pairwise inter-view learning, which extracts task-relevant modality-specific and shared information across modalities}
    \label{cookie_method}
\end{figure}
% \vspace{-1em}

\subsection{Intra-view learning} 
Intra-view contrastive learning extracts representative features of each region within each modality by using other regions as negative samples and an augmentation pair as a positive sample, as shown in the intra-view learning section of Figure~\ref{cookie_method}. Through intra-view learning, we pretrain each modality's encoder to provide a more robust initialization than random initialization. In the following paragraphs, we introduce augmentation methods for each modality. 
% Intra-view learning with contrastive learning captures distinctive, modality-specific features by emphasizing the uniqueness of each region by maximizing discrepancies, as shown in Figure~\ref{cookie_method}. We pretrain intra-view learning to output a better initial stage for the encoder. Specifically, we generate augmentation pairs by avoiding significantly altering or destroying the original representations~\cite{factorcl}. 

\textbf{POIs and AOIs.} To simulate real-world changes, we apply minimal augmentation methods that help \modelname remain consistent with the original POIs and AOIs for $\mathcal{U}$.
Our approach includes three augmentations similar to~\cite{tkde} for each type of POIs and AOIs (e.g., parks, schools): (1) random addition, (2) random removal, and (3) random replacement with a low probability (0.1). We use Multi-Layer Perception (MLP) as the encoder to learn embeddings from raw feature vectors. We perform intra-view learning for POIs and AOIs modality separately.

\textbf{Satellite Imagery.} 
To help \modelname capture core image features while maintaining original semantics, we create an augmented image as a positive pair and use images from other regions as negatives, inspired by recent success in self-supervised image learning~\cite{simclr}.
For the augmentation, we include random flipping, random color changing, and Gaussian noise but exclude random cropping, which modifies the original semantics. We use a pretrained ResNet-50 backbone as the encoder to extract image features. 

\textbf{Building Footprints.}
To preserve 2-D polygonal building shapes and spatial locations, we encode individual building footprints into visual features using a pretrained ResNet-18. Following the approach in~\cite{li2023urban}, we apply random flips and rotations to each building, making the features invariant to changes in size and orientation.
Further, we aggregate building features into $\mathcal{U}$ for capturing region-level representations. 
We introduce a region-level augmentation by randomly dropping 10\% of building features during aggregation for a positive pair, while using features from other regions as negative pairs. We then use a MLP encoder then extracts the region-level features, and contrastive learning is applied using the augmented building features.

% We utilize building footprints, which include 2D polygonal shapes. Inspired by~\cite{li2023urban}, we then preserve 2D polygons to image using Resnet-18 to extract distinct building features for preserving the size and rotation of each building. 
% To capture the representation of building features at the region level, we generate a positive pair by randomly dropping 10\% of building features within each region and negative pairs from other regions. We then use an MLP encoder to extract region-level features and apply contrastive learning with the augmented building features.

\subsection{Preliminaries: Factorized Contrastive Learning (FactorCL)}\label{factorcl:challenge}
% how factorcl achieve what they did and weakness.
\textbf{Background.} 
FactorCL~\cite{factorcl} demonstrates how to capture task-relevant shared and unique information between two modalities by decomposing task-relevant and task-irrelevant semantics in both supervised and self-supervised learning. 
For shared information between modalities $i$ and $j$ ($S_{z_{ij}}$), FactorCL learns task-relevant shared information by maximizing lower bound of $I_{NCE}(x_i, x_j)$~\cite{oord2018representation} and removes task-irrelevant information by minimizing upper bound of the conditional mutual information, $-I_{CLUB}(x_i, x_j | x_i^\prime, x_j^\prime)$~\cite{clubloss}, where $^\prime$ refers to augmentation pair of each modality. For unique information, FactorCL captures task-relevant unique feature by maximizing lower bound of $I_{NCE}(x_i, x_i^\prime)$ while removing non-unique information by minimizing upper bound of $-(I_{CLUB}(x_i, x_j)$ $- I_{NCE}(x_i; x_j | x_i^\prime, x_j^\prime))$. 
% Note that FactorCL assumes unimodal augmentation, $x^{\prime}_i$, as a proxy of task label $y$ in self-supervised learning, following~\cite{tian2020makes}. 
Specifically, $I_{NCE}$ is defined as: 
\begin{align}\label{eq:infoNCE}
    &I_{NCE}(x_i;x_j|x_i^{\prime};x_j^{\prime})  \nonumber \\
    & \!\!\!\!\!\!=\mathbb{E}_{p(x_i^{\prime}, x_j^{\prime})} \!\!\left[ \mathbb{E}_{\substack{x_i, x_j^{+}\sim p(x_i, x_j^{+} | x_i^\prime, x_j^\prime) \\ x_j^- \sim p(x_j^- | x_i^\prime, x_j^\prime)}}\left[ \log\frac{\exp(f(x_i, x_j^{+}, x_i^{\prime}, x_j^{\prime}))}{\sum \exp(f(x_i, x_j^{-}, x_i^{\prime}, x_j^{\prime}))}\right]\right],
\end{align}
where $x_j^{+}$ and $x_j^{-}$ are the positive and negative augmentations of $x_j$ given knowledge of $x_i^{\prime}$ and $x_j^{\prime}$ and $f(\cdot)$ is an encoder. 
% where $x_i^{\prime}$ and $x_j^{\prime}$ are the positive augmentation pair of $x_i$ and $x_j$ modality, $x_j^{+}$ and $x_j^{-}$ are the positive (e.g., an augmented data sample of the region) and negative augmentations (e.g., the same modality sample of other regions) of $x_j$ given knowledge of $x_i^{\prime}$ and $x_j^{\prime}$, $f(\cdot)$ is an encoder, and the summation in the denominator is with respect to negative samples $x_j^-$. We note that $x_j^{\prime}$ and $(x_i,x_j^+)$ are distributed according to $x_j^{\prime} \sim p(x_j^{\prime})$ and $(x_j,x_j^{\prime})\sim p(x_i, x_j^+|x_i^{\prime}, x_j^{\prime})$ (for more details, see~\cite[eq.~(15)]{factorcl}).
Thus, the maximum mutual information can be derived by the lower bound i.e., $I(x_i; x_j) \geq -I_{NCE}(x_i; x_j)$~\cite{oord2018representation}.

Similarly, $I_{CLUB}$ aims to remove task-irrelevant information by minimizing the upper bound of the mutual information between $x_i$ and $x_j$~\cite[Theorem 3.1.]{clubloss} (i.e., $I_{CLUB}(x_i; x_j) \geq I(x_i; x_j)$). $I_{CLUB}$ is defined as:
\begin{align}\label{eq:club}
    & I_{CLUB}(x_i;x_j|x_i^{\prime};x_j^{\prime}) \nonumber \\
    & \! = \mathbb{E}_{p(x_i^{\prime}, x_j^{\prime})} \left[ \mathbb{E}_{x_i, x_j^{+} \sim p(x_i, x_j^{+} | x_i^\prime, x_j^\prime)} \left[f(x_i, x_j^{+}, x_i^{\prime}, x_j^{\prime})\right] \right.  \nonumber \\
    & \qquad\qquad\quad \left.- \mathbb{E}_{\substack{x_i \sim p(x_i | x_i^\prime, x_j^\prime) \\ x_j^- \sim p(x_j^- | x_i^\prime, x_j^\prime)}} \left[ f(x_i, x_j^{-}, x_i^{\prime}, x_j^{\prime}) \right] \right],
\end{align}
where $f$ refers to the same encoder used in $I_{NCE}$.

\noindent \textbf{Challenge: Extending FactorCL to three modalities.}
We demonstrate how to expand FactorCL to multiple modalities in multimodal region representation learning. We extend FactorCL to handle three modalities to find modality-specific information $U_{z_i}$ of $z_i$, shared information between two modalities $z_i$ and $z_j$ as $S_{z_{ij}}$, and shared information across three modalities as $S_{z_{ijk}}$. Here, we define $z_i$ as the representation of the $x_i$ modality using a backbone encoder. Generalizing each term is followed by
\begin{align}
    U_{z_i} & = \arg\max_{}I(z_i; z^{\prime} |z_j, z_k), \\
    S_{z_{ij}} & = \arg\max_{}I(z_i; z_j; z^{\prime} | z_k), \\
    S_{z_{ijk}} & = \arg\max_{}I(z_i; z_j; z_k; z^{\prime}),
\end{align} 
where $z^{\prime}$ represents a concatenation of augmentation pairs~\cite{sordoni2021decomposed} relevant to the mutual information of modalities in each term. For instance, in $I_{NCE}(z_i; z_j, z_k | z^{\prime})$ in Equation~\ref{factorcl:cha:eq1_fac}, $z^{\prime}$ consists of a concatenation of augmentation pairs from all three modalities ($z_i^{\prime}, z_j^{\prime}, z_k^{\prime}$). Each objective (i.e., $U_{z_i}$, $S_{z_{ij}}$, and $S_{z_{ijk}}$) can be further decomposed using interaction information term:
\begin{align}
    U_{z_i} & = I_{NCE}(z_i; z^{\prime}) - I_{CLUB}(z_i; z_j, z_k) \nonumber \\
    & \quad\quad + I_{NCE}(z_i; z_j, z_k | z^{\prime}), \label{factorcl:cha:eq1_fac}\\
    S_{z_{ij}} & = I_{NCE}(z_i; z_j| z_k) - I_{CLUB}(z_i; z_j | z_k, z^{\prime}), \label{factorcl:cha:eq2_fac} \\
    S_{z_{ijk}} & = I_{NCE}(z_i; z_j ; z_k) - I_{CLUB}(z_i; z_j; z_k | z^{\prime}),  \nonumber \\
    & = I_{NCE}(z_i; z_j) - I_{CLUB}(z_i; z_j | z_k)  \nonumber \\
    & \quad\quad - I_{CLUB}(z_i; z_j | z^{\prime})  \nonumber \\
    & \quad\quad + I_{NCE}(z_i; z_j | z^{\prime}, z_k),  \label{factorcl:cha:eq2_fac}
\end{align}
where $U_{z_i}$, $S_{z_{ij}}$, and $S_{z_{ijk}}$ use $I_{NCE}$ in Equation~\ref{eq:infoNCE} to capture task-relevant information and $I_{CLUB}$ in Equation~\ref{eq:club} to remove task-irrelevant information.
Extending FactorCL to handle more than two modalities increases the complexity due to the additional objectives, such as $S_{z_{ijk}}$. For instance, with four modalities, the learning objectives account for shared information across various combinations, such as $S_{z_{123}}$, $S_{z_{124}}$, $S_{z_{234}}$, and $S_{z_{1234}}$, which leads to a significant increase in the number of mutual information terms to optimize.
% with four modalities, learning objectives for shared information among up to four modalities must be considered, including $S_{123}$, $S_{124}$, $S_{234}$, $S_{1234}$, which leads to a significant increase in the number of mutual information terms to optimize.
% Although higher-order combinations can capture additional details, they often introduce redundancy and computational overhead.

% The complete form of the expanded FactorCL increases the number of learning objectives, such as $S_{z_{ijk}}$. With four modalities, the shared information among multiple modalities ($S_{z_{ijk}}$, $S_{z_{ijkl}}$) must be included, leading to objectives like $U_1$, $U_2$, $U_3$, $U_4$, $S_{12}$, $S_{13}$, $S_{14}$, $S_{23}$, $S_{24}$, $S_{34}$, $S_{123}$, $S_{124}$, $S_{234}$, $S_{1234}$. Each objective decomposes into mutual information terms, including multiple $I_{NCE}$ and $I_{CLUB}$ loss terms. The final embedding is a concatenation of all linear heads corresponding to each loss term. Higher-order combinations, such as $S_{z_{ijk}}$ and $S_{z_{ijkl}}$, might capture some additional details but often results in redundancy and increased complexity. 
% Consequently, as the number of modalities increases, the number of learning objectives increases. 
% among three and four modalities must be included, along with the unique and shared information between two modalities. As the number of modalities grows, the dimensionality of the final embeddings also increases due to the expanded set of learning objectives. Therefore, the increased dimensionality makes capturing shared and unique information difficult when extending FactorCL to multiple modalities.

\subsection{Pairwise inter-view learning} 
To mitigate the redundancy and complexity associated with high-order combinations, we propose a pairwise inter-view learning approach, as described in Figure~\ref{cookie_method}. Our method captures task-relevant shared information while preserving the unique information across all modalities by focusing on pairwise interactions. 
Our approach defines unique and shared information using a generalized form:
% Existing contrastive learning methods risk over-fitting to the shared information between modalities~\cite{wang2022rethinking}, which potentially causes unique information to diminish due to the emphasis on mutual information between modalities.
% % This challenge is further compounded when capturing shared information across multiple modalities ($N \geq 3$). 
% To address these challenges, we propose a pairwise fusion method in inter-view learning that captures shared information while preserving unique information across all modalities. 
% In particular, we define the general form of unique and shared information as follows:
\begin{align}
    U_{z_i} & = \arg\max_{}I(z_i; z^{\prime} |z_j) \nonumber \\
    &= I_{NCE}(z_i; z_i^{\prime}) - I_{CLUB}(z_i, z_j)  \nonumber \\
    & \quad\quad + I_{NCE} (z_i;z_j|z_i^{\prime},z_j^{\prime}), \label{method:U}\\
    S_{z_{ij}} & = \arg\max_{}I(z_i; z_j; z^{\prime}) \nonumber \\
    &= I_{NCE}(z_i; z_j) - I_{CLUB}(z_i, z_j | z_i^{\prime}, z_j^{\prime}),\label{method:S}
\end{align}
where $z_i$ and $z_j$ represent all possible modality pairs. $U_{z_i}$ is unique information for each modality and $S_{z_{ij}}$ shows shared information between two modality pairs. 
This pairwise approach minimizes the number of learning objectives, avoiding the repetition of information already captured through the pairwise interactions.
% This pairwise approach limits the number of learning objectives, effectively avoiding the repetition of information that has already been captured through simpler pairwise interactions reducing redundancy. 
For example, with three modalities, our method requires six objectives ($U_{z_1}$, $U_{z_2}$, $U_{z_3}$, $S_{z_{12}}$, $S_{z_{13}}$, $S_{z_{23}}$), while extending FactorCL results in seven, including those six objectives with the high-order term, $S_{z_{123}}$. The difference becomes more significant as the number of modalities increases: with four modalities, our approach uses 10 objectives ($U_{z_1}$, $U_{z_2}$, $U_{z_3}$, $U_{z_4}$, $S_{z_{12}}$, $S_{z_{13}}$, $S_{z_{14}}$, $S_{z_{23}}$, $S_{z_{24}}$, $S_{z_{34}}$) compared to FactorCL’s 14 (additionally including $S_{z_{123}}$, $S_{z_{124}}$, $S_{z_{234}}$, $S_{z_{1234}}$), and with five modalities, our approach uses 15 objectives compared to FactorCL’s 25.
Additionally, each objective is further decomposed by several InfoNCE and CLUB losses, which scale quadratically with the number of modalities, following $O(n^2)$, whereas FactorCL scales exponentially, following $O(2^n)$. 

\subsection{\modelname objectives}
In the final stage, we integrate the intra-view learning loss and pairwise inter-view learning loss in \modelname. The joint objective function is expressed as:
\begin{align}
    \mathcal{L} 
    &= \mathcal{L}_{intra} + \mathcal{L}_{inter} \\
    &= (\mathcal{L}_{z_{1}} + ... + \mathcal{L}_{z_{i}}) + (U_{z_i} + S_{z_{ij}}),
\end{align}
where $\mathcal{L}_{intra}$ refers to the intra-view learning loss for each modality $i$ (represented by $\mathcal{L}_{z_{i}}$), and $\mathcal{L}_{inter}$ refers to the inter-view learning loss, which captures both the unique information $U_{z_i}$ and the shared information $S_{z_{ij}}$ between modality $i$ and other modalities $j$. After training \modelnamex, we apply a random forest classifier for classification tasks and MLP for regression tasks. Section~\ref{exp:downstream} provides further details on the downstream tasks.

% I think you need to talk about what features to concatenate and use RF to do prediction here cuz in 4.4.1, you are talking about "The final embedding is obtained by concatenating all four learned embeddings."


==> backup/preliminary.tex <==
\section{Problem Statement}
\begin{definition}[Urban regions] A city can be divided into distinct regions, defined as $\mathcal{U} = \{ u_1, ... , u_n\}$, where $n$ is the number of regions. We use census tracts and ward-level boundaries as partitions.
\end{definition}

\begin{definition}[Urban attributes]
A region is characterized by a set of modalities, denoted as $\mathcal{X} = \{x_1,..., x_m\}$, where each $x_m$ represents a distinct modality such as POI, AOI, or satellite imagery.
\end{definition}

% \begin{problemstate}[Urban region representation learning]
\textbf{Problem Statement (Urban region representation learning).}
Given a set of regions $\mathcal{U}$, we aim to learn representations from the modalities $\mathcal{X}$. The learned region embeddings are denoted as $E = \{ e_1, ..., e_n\}$, where $e_i \in \mathbb{R}^k$ represents the embedding for region $i$, and $k$ is the embedding dimension.
% \end{problemstate}

% \begin{definition}[Unimodal augmentation.]\label{opt_aug}
% In self-supervised learning, the task label $Y$ is not provided. Alternatively, $y$ can be replaced with task-relevant semantics for each modality, $x^{\prime}_i$, using unimodal augmentation. 
% As stated in~\cite{tian2020makes, factorcl}, $x^{\prime}_i$ serves as an optimal augmentation when $I(x_i;x^{\prime}_i) = I(x_i;y)$. 
% % ensuring task-relevant information without irrelevant noise. 
% In this paper, we use $x^{\prime}_i$ instead of $Y$ for self-supervised region representation learning.
% \end{definition}

% \begin{definition}[Task-relevant unique and shared information]\label{def_mi} 
% Followed by Definition~\ref{opt_aug}, we define task-relevant semantics with augmentation pair of $X$, $Z^{\prime}$. We then define task-relevant unique information as follows, 
% \begin{subequations}
% \begin{align}
%     U_{Z_1} & = \arg\max_{}I(Z_1; Z^{\prime} |Z_2), \label{def:eq1} \\
%     S_{Z_{12}} & = \arg\max_{}I(Z_1; Z_2; Z^{\prime}), \label{def:eq2}
% \end{align}
% \end{subequations}
% where $Z_1$ and $Z_2$ are the input modality semantics, and $Z^{\prime}$ is the augmentation pair. Equation~(\ref{def:eq1}) represents maximizing task-relevant unique information, while Equation~(\ref{def:eq2}) is to maximize task-relevant shared information.
% \end{definition}

% \begin{definition}[Task-relevant unique and shared information]\label{def_mi} 
% We define task-relevant unique and shared information in the case of three modalities using conditional mutual information, inspired by~\cite{factorcl}. 
% \begin{align}\label{eq:def}
%     & I(Z_1, Z_2, Z_3 | Z^{\prime}) \nonumber \\
%     & = \underbrace{I(Z_1; Z^{\prime}|Z_2, Z_3) + I(Z_2; Z^{\prime}|Z_1, Z_3) + I(Z_3; Z^{\prime}|Z_1, Z_2)}_{\text{Task-relevant unique information}} \nonumber \\
%     & + \underbrace{I(Z_1; Z_2; Z^{\prime}| Z_3) + I(Z_1; Z_3; Z^{\prime}| Z_2) + I(Z_2; Z_3; Z^{\prime}| Z_1)}_{\text{Task-relevant shared information between two modals}} \nonumber \\
%     & + \underbrace{I(Z_1; Z_2; Z_3; Z^{\prime}),}_{\text{Task-relevant shared information between three modals}}
% \end{align}
% where task-relevant unique information is existed in between one modality and task-relevant semantic $Z^{\prime}$ and task-relevant shared information is existed in between two or three modalities and $Z^{\prime}$. 
% % We further decompose the conditional mutual information using information interaction to learn the pair of representation. 
% We also illustrate how each task-relevant representation can be bounded in Figure~\ref{cookie_ex}. We further explain how we decompose the shared information between multiple modalities to conditional mutual information in Method. 
% % $\mathcal{I}(Z_{S}, Z_{A}; Z^{\prime} | Z_{P})$ denotes the mutual information between $(Z_{S}, Z_{A})$ and $Z^{\prime}$, given by $Z_{P}$. 
% % This implies that only the common information between $(Z_{S}, Z_{A})$ and $K$ is considered.
% \end{definition}

% % task-relevant shared information
% \begin{definition}[Task-relevant unique information]\label{def_uni} \textit{Task-relevant unique information represents the unique semantics where one input modality shares regarding as $K$. In Figure~\ref{cookie_ex}, $\mathcal{I}(Z_{S}; Z^{\prime} | Z_{A}, Z_{P})$ denotes the mutual information between $Z_{S}$ and $Z^{\prime}$, given by $Z_{A}$ and $ Z_{P}$.}
% \end{definition}


==> backup/relatedwork.tex <==
\section{Related Work}
\subsection{Region Representation Learning}
% multi-view concatenation
Recent methods have focused on learning region representations from unlabeled geospatial data by leveraging multiple data sources. 
CGAL~\cite{zhang2019unifying} combines taxi trajectories and POI to construct regional structures and capture spatial autocorrelation between regions.
RegionEncoder~\cite{jenkins2019unsupervised} extracts representations from satellite imagery, POI, and human mobility data using a graph-based approach, then concatenates these learned representations to form the final region representation. 
MV-PN~\cite{fu2019efficient} constructs geographical distance and human mobility views using an intra-region POI network by leveraging a spatial autocorrelation between regions. 
MVURE~\cite{mvure} employs a graph-attention network to learn region relationships from POI and human mobility data, fusing the learned representations through a weighted sum method.
Although these methods utilize a multi-view approach in region representation learning, their final representations rely on simple concatenation or the weighted sum to fuse modal-specific representations, which overlook inter-view correlations across modalities.

% multi-view attention
To leverage correlations between representations from multiple modalities, recent approaches exploit attention-based mechanisms to fuse the learned representations. 
MGFN~\cite{wu2022multi_mgfn} integrates mobility graphs by identifying temporal mobility patterns and expanding the patterns into multiple views. This approach then employs multi-level cross-attention mechanisms to capture detailed region representations.
HAFusion~\cite{sun2024urban} extracts view-specific representations using POIs, human mobility, geographic boundary, and land use features. HAFusion then combines these representations using region-wise and view-wise attention fusion techniques to emphasize the important features across regions and within each modality. 
HREP~\cite{zhou2023heterogeneous} constructs a heterogeneous graph using human mobility, POIs, and geographic neighbors of regions and blends them using an attention mechanism to learn region representation. 

% multi-view contrastive learning
However, these approaches fail to align representations between modalities because they focus on key features within each modality using attention-based methods. 
KnowCL~\cite{liu2023knowledge} constructs a knowledge graph by spatial location, POI, and human mobility data. KnowCL then fuses the knowledge graph with geospatial visual features (e.g., street view imagery and satellite imagery) through contrastive learning. 
RegionDCL~\cite{li2023urban} learns region representations by fusing building footprints and POI data through building group-level and region-level contrastive learning. 
ReMVC~\cite{tkde} extracts unique region features from POIs and human mobility during intra-view learning and incorporates representation alignment between these modalities via inter-view contrastive learning. Similarly, \citet{li2024urban} captures intra- and inter-view relationships using POIs and human mobility data and preserving the original features of each modality through feature reconstruction.
While contrastive learning in inter-view fusion helps capture shared information and align modalities, this method often heavily focuses on sharing information, which may overlook preserving modality-specific features during inter-view learning. 
In contrast, \modelname aims to capture both task-relevant shared and unique information when aligning multiple modalities in inter-view learning across various modalities. 

% Tile2Vec~\cite{jean2019tile2vec} extracts region embeddings from satellite images using geographic adjacency to predict poverty.
% ZE-Mob~\cite{yao2018representing} utilizes taxi trajectory data to discover region correlations and generate region representations using a graph-based model. 
% MGFN~\cite{wu2022multi} integrates mobility graphs with spatiotemporal similarity to capture mobility patterns and employs multi-level cross-attention mechanisms for detailed region representations.
% Recent methods propose to learn region representations from unlabeled geospatial data by utilizing multiple data sources. 
% MVURE~\cite{mvure} learns region relationships using POI and human mobility data through a graph-attention network then fuse each learned representation by weighted sum approach. 
% Wang et al.~\cite{wang2017region} construct flow and spatial graphs by using taxi trajectory data along with POI.


% One category of unsupervised region representation learning methods use graph structure to represent region relationships using human mobility or spatial proximity. ZE-Mob~\cite{yao2018representing} employs a graph-based model to identify region relationships and generate region representations. Similarly, Wang et al.\citet{wang2017region} and CGAL~\cite{zhang2019unifying} construct multiple graphs to capture the regional structure and the spatial autocorrelation between regions. However, these methods heavily rely on the graph-based method, which is challenging in applicability in regions where the graph-based data is not available. 
% % While these methods demonstrate effectiveness in evaluating on predicting various downstream tasks, they fail to incorporate intra-view learning for each modality.

% Recent approaches integrate additional data sources to capture unique region representation and relationships between regions.
% MGFN~\cite{wu2022multi_mgfn} combines mobility graphs with spatiotemporal similarity to capture mobility patterns and employs multi-level cross-attention mechanisms for detailed region representations.
% MVURE~\cite{mvure} learns region relationships using POI and human mobility data through a graph-attention network. 
% HAFusion~\cite{sun2024urban} extracts a view-specific representation using POIs, human mobility, geographic boundary, and land use features, then fuses each modality using the attention-based model. 
% HREP~\cite{zhou2023heterogeneous} constructs a heterogeneous graph using human mobility, POI data, and geographic neighbors of regions and fuses them using an attention mechanism to learn region representation. 

% However, these approaches rely on attention-based method for fusion, which fails to align representation between modalities. ReMVC~\cite{tkde} extracts unique region features from POIs and human mobility during intra-view learning and incorporates semantic alignment between these modalities in inter-view learning through contrastive learning. \citet{li2024urban} capture intra- and inter-view relationships using POIs and human mobility data while preserving the original semantics of each modality through feature reconstruction.
% Although contrastive learning-based methods have demonstrated effectiveness in representation alignment, they often overlook preserving unique information during inter-view learning.

% Moreover, some studies utilize positive and negative pairs in region representation within modality. 
% Urban2Vec~\cite{wang2020urban2vec} integrates street view imagery and POI descriptions from Yelp reviews using triplet loss within each modality to leverage spatial autocorrelation. 
% RegionDCL~\cite{li2023urban} incorporates POI and building footprints to learn region representations by optimizing region and building group similarities through contrastive learning.
% However, these methods has a lack of aligning the shared information between modalities. 

\subsection{Contrastive Learning}
Contrastive learning aims to derive unique representations from unlabeled data by constructing positive and negative pairs~\cite{contrastivesurvey} (e.g., optimizing through noise contrastive estimation (NCE)). SimCLR~\cite{simclr} shows a promising performance by generating positive pairs using image augmentation methods, enabling the model to discern meaningful features by maximizing similarity between transformed images and minimizing it with dissimilar ones~\cite{simclr}. Furthermore, CLIP~\cite{clip} shows promising results in aligning the image and text modalities in a joint space through contrastive learning, which effectively aligns representation between image-text.

Although aligning the modalities into a single space is considered the common information between modalities, this type of approaches does not account for unique information potentially important for representation learning. 
To address this limitation, FactorCL~\cite{factorcl} extracts semantics by capturing mutual and unique information between two modalities, demonstrating the effectiveness of extracting complementary information in representation learning. However, the computational complexity increases when more than two modalities are incorporated. In comparison, \modelname effectively captures both unique and shared information through a pairwise inter-view fusion approach, thereby reducing the number of learning objectives.

% through the noise contrastive estimation (NCE). This approach demonstrates effectiveness in computer vision by using augmented image transformations to generate positive pairs~\cite{simclr}. This method allows the model to discern meaningful features by maximizing the similarity between transformed images and minimizing it with dissimilar images. Furthermore, CLIP~\cite{clip} shows promising results in aligning the image and text modalities in a joint space through contrastive learning, which effectively transfers knowledge between modalities. 

==> backup/results.tex <==
\section{Results}

\begin{table*}[h]
\centering
\caption{Compare \modelname to baselines on population density and crime rate prediction in NYC. $\downarrow$ means the smaller value is the better and $\uparrow$ is the opposite. We bold the best result and underscore the second best. The modalities used in the models include POI ($\mathcal{P}$), AOI ($\mathcal{A}$), satellite imagery ($\mathcal{S}$), building footprints ($\mathcal{B}$), mobility ($\mathcal{M}$) and  knowledge graph ($\mathcal{KG}$).}
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular}{cccccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Population}} & \multicolumn{3}{c}{\textbf{Crime}}\\
\cmidrule(rl){3-5} \cmidrule(rl){6-8} 
\textbf{Methods} & \textbf{Modalities} & {MAE} $\downarrow$ & {RMSE} $\downarrow$ & {R2} $\uparrow$ & {MAE} $\downarrow$ & {RMSE} $\downarrow$ & {R2}$\uparrow$\\
\midrule
% Urban2Vec & Streetview, text & 5328.38$\pm$200.58  & 7410.42$\pm$261.89  & 0.522$\pm$0.028 & 124.432$\pm$5.168 & 185.318$\pm$14.252 & 0.151$\pm$0.058 \\
% MVURE & MOB + POI & 6557.12$\pm$265.30 & 8307.58$\pm$329.44 & 0.404$\pm$0.034 & 114.548$\pm$2.545 & 161.039$\pm$10.128 & 0.242$\pm$0.035  \\
MGFN & $\mathcal{M}$ & 6754.58$\pm$201.13 & 8989.14$\pm$312.71 & 0.331$\pm$0.050 & 116.08$\pm$4.40 & 161.94$\pm$9.86 & 0.231$\pm$0.043   \\
% RegionDCL & $\mathcal{B}$ + $\mathcal{P}$ & 50.20$\pm$2.16 & 69.60$\pm$2.82 & 0.575$\pm$0.040 & 11.52$\pm$0.122 & 17.60$\pm$1.180 & 0.177$\pm$0.022  \\ %\midrule
MVURE & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{M}$ & 5295.00$\pm$101.72 & 7065.08$\pm$122.91 & 0.545$\pm$0.014    & 108.60$\pm$5.01 & 151.87$\pm$13.46 & 0.278$\pm$0.043 \\ 
RegionDCL & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 4891.96$\pm$103.11 & 6890.84$\pm$164.84 & 0.568$\pm$0.013     & 106.00$\pm$2.36 & 163.71$\pm$15.17 & 0.29$\pm$0.034 \\
FactorCL & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 4858.29$\pm$211.66 & 6482.78$\pm$289.20 & 0.590$\pm$0.028 & 104.522$\pm$4.00 & 152.28$\pm$14.10 & 0.306$\pm$0.043 \\
% 
Urban2Vec & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ & 4760.06$\pm$191.45 & 6497.80$\pm$395.89 & 0.614$\pm$0.053 & 104.95$\pm$3.49 & 159.28$\pm$12.24 & 0.326$\pm$0.040 \\ 
ReMVC & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ & 7321.98$\pm$122.16 & 9189.99$\pm$196.61 & 0.19$\pm$0.016 & 119.68$\pm$3.28 & 166.94$\pm$12.16 & 0.182$\pm$0.039 \\ 
 \midrule  \midrule 
% 
% \color{blue}\modelname-PLANET& $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 5254.45$\pm$200.51 & 7197.56$\pm$282.74& 0.525$\pm$0.03 & 114.8$\pm$4.05 & 166.67$\pm$13.43 & 0.248$\pm$0.04  \\
% \color{purple}\modelname-intra& $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 4686.19$\pm$216.06 & 6256.38$\pm$312.36 & 0.624$\pm$0.033 & 105.68$\pm$3.25 & 146.041$\pm$11.44 & 0.346$\pm$0.026  \\
\modelname& $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 4627.80$\pm$163.49 & \underline{6306.03$\pm$296.37} & \underline{0.630$\pm$0.033} & 105.47$\pm$3.17 & 149.54$\pm$11.40 & 0.322$\pm$0.030  \\
% \color{cyan}{\modelname-no intra} & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 4874.20$\pm$131.63 & 6420.22$\pm$190.87 & 0.600$\pm$0.022 & 111.90$\pm$2.88 & 165.15$\pm$12.36 & 0.275$\pm$0.029  \\ 
% \color{cyan}{\modelname-no intra} & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 4691.68$\pm$68.93 & 6497.81$\pm$139.12 & 0.611$\pm$0.017 & 102.31$\pm$4.56 & 146.33$\pm$14.05 & 0.336$\pm$0.036  \\
\modelname & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & \underline{4562.71$\pm$43.51} & 6316.58$\pm$89.46 & 0.627$\pm$0.009 & \underline{102.28$\pm$4.32} & \textbf{147.35$\pm$13.55} & \underline{0.346$\pm$0.030}  \\
% \color{cyan}{\modelname-no intra} & $\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & \textbf{4096.22$\pm$159.03} & \textbf{5824.79$\pm$197.98} & \textbf{0.695$\pm$0.019} & \textbf{98.92$\pm$2.30} & \textbf{145.35$\pm$14.35} & \textbf{0.375$\pm$0.039} \\ 
\modelname & $\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & \textbf{4102.23$\pm$124.62} & \textbf{5584.12$\pm$221.17} &  \textbf{0.698$\pm$0.017} & \textbf{99.2$\pm$1.65}& \underline{148.52$\pm$11.37} & \textbf{0.377$\pm$0.017} \\ \midrule \midrule 
KnowCL (log) & $\mathcal{S}$ + $\mathcal{KG}$ & - & 0.612 & 0.153 & - & 0.622 & 0.536  \\ 
\modelname (log) & $\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$  & - &  0.399 & 0.557 & - & 0.621 & 0.534 \\ \bottomrule
% COOKIE & SAT + POI + AOI + (BF)\textcolor{red}{concat bf} & 4300.936$\pm$120.867 & 5926.12$\pm$157.301 & 0.675$\pm$0.017 &  
  % \\ \bottomrule
\end{tabular}
\label{table_result_1}
\end{adjustbox}
\end{table*}




\begin{table*}[h]
\centering
\caption{Compare \modelname to baselines on Greenness and land use classification in NYC.}
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular}{cccccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Greenness}} & \multicolumn{3}{c}{\textbf{Land Use}}\\
\cmidrule(rl){3-5} \cmidrule(rl){6-8} 
\textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {L1}$\downarrow$ & {KL}$\downarrow$ & {Cosine}$\uparrow$\\
\midrule
MGFN & $\mathcal{M}$ & 3.949$\pm$0.187 & 5.032$\pm$0.255 & 0.094$\pm$0.023 & 0.530$\pm$0.012 & 0.334$\pm$0.011 & 0.875$\pm$0.006\\
MVURE & $\mathcal{M} + \mathcal{P} + \mathcal{B}$ & 3.723$\pm$0.201 & 4.875$\pm$0.259 & 0.183$\pm$0.039 & 0.526$\pm$0.008 & 0.337$\pm$0.011 & 0.872$\pm$0.006 \\ 
RegionDCL &$\mathcal{B} + \mathcal{P} + \mathcal{A}$& 3.481$\pm$0.176 & 4.574$\pm$0.254 & 0.290$\pm$0.032 & 0.488$\pm$0.005 & 0.273$\pm$0.007 & 0.893$\pm$0.005 %L2: 0.282±0.004 
\\ 
% RegionDCL &$\mathcal{B} + \mathcal{P} + \mathcal{A}$& 3.481$\pm$0.176 & 4.574$\pm$0.254 & 0.29$\pm$0.032 & \textbf{0.412$\pm$0.012} & 0.241$\pm$0.02 & \underline{0.911$\pm$0.006} \\ 
FactorCL & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$  & 3.527$\pm$0.194 & 4.457$\pm$0.268 & 0.260$\pm$0.025 & 0.477$\pm$0.010 & 0.280$\pm$0.017 & 0.893$\pm$0.006 \\
% l2: 0.271±0.006
% Urban2Vec &$\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$&  3.373$\pm$0.163 & 4.423$\pm$0.239 & \textbf{0.337$\pm$0.028} & \underline{0.422$\pm$0.017} & 0.241$\pm$0.019 & 0.91$\pm$0.006 \\
Urban2Vec &$\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$&  3.373$\pm$0.163 & 4.423$\pm$0.239 & \textbf{0.337$\pm$0.028} & \underline{0.421$\pm$0.007} & \textbf{0.223$\pm$0.007} & \textbf{0.915$\pm$0.006} \\
ReMVC & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ & 4.051$\pm$0.192 & 5.151$\pm$0.240 & 0.068$\pm$0.026 & 0.608$\pm$0.029 & 0.475$\pm$0.027 & 0.831$\pm$0.012 \\ 
% l2: 0.244, 
% MVURE & MOB + POI & 4.067$\pm$0.272 & 5.186$\pm$0.338 & 0.048$\pm$0.029 & 0.542$\pm$0.014 & 0.329$\pm$0.014 & 0.872$\pm$0.006 \\
% RegionDCL & BF + POI &  \underline{3.433$\pm$0.198} & \underline{4.547$\pm$0.298} & \underline{0.298$\pm$0.03} & \underline{0.418$\pm$0.010} & \underline{0.229$\pm$0.008} & \underline{0.912$\pm$0.004}   \\ \midrule
% FactorCL & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & & & & & &  \\
\midrule \midrule
% Urban2Vec\color{red}{Yijun} & SAT+ POI + AOI & 3.373$\pm$0.163 & 4.423$\pm$0.239
%  & 0.337$\pm$0.028 & 0.422$\pm$0.017 & 0.241$\pm$0.019 & 0.91$\pm$0.006 \\\midrule \midrule   
% \color{blue}\modelname-PLANET& $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 3.697$\pm$0.206 & 4.744$\pm$0.255 & 0.204$\pm$0.018 & 0.5624$\pm$0.0154 & 0.3429$\pm$0.0039 & 0.8616$\pm$0.003  \\
% \color{purple}\modelname-intra& $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 3.634$\pm$0.198 & 4.575$\pm$0.254 & 0.224$\pm$0.012 & 0.453$\pm$0.015 & 0.256$\pm$0.015 & 0.902$\pm$0.005  \\
\modelname& $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 3.573$\pm$0.157 & 4.583$\pm$0.221 & 0.251$\pm$0.017 & 0.424$\pm$0.010 & 0.236$\pm$0.060 & \underline{0.913$\pm$0.003} 
%L2;0.2446, 0.0047
\\ 
% \modelnamex & $\mathcal{S} + \mathcal{P} + \mathcal{A}$  & 3.627$\pm$0.165 & 4.714$\pm$0.237 & 0.234$\pm$0.035 & 0.455$\pm$0.009 & 0.250$\pm$0.009 & 0.906$\pm$0.004  \\ 
% \modelnamex & $\mathcal{B} + \mathcal{P} + \mathcal{A}$  & 3.53$\pm$0.174 & 4.49$\pm$0.267 & 0.259$\pm$0.015 & 0.594$\pm$0.008 & 0.379$\pm$0.006 & 0.851$\pm$0.004   \\ 
\modelname& $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & \underline{3.444$\pm$0.175} & \underline{4.371$\pm$0.246} & 0.292$\pm$0.011 & 0.442$\pm$0.010 & 0.267$\pm$0.080 & 0.901$\pm$0.003 %L2;0.25222, 0.0035
\\
% \modelnamex & $\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A}$  & \textbf{3.398$\pm$0.173} & \textbf{4.266$\pm$0.27} & \textbf{0.313$\pm$0.022} & \textbf{0.39$\pm$0.016} & \textbf{0.203$\pm$0.011} & \textbf{0.923$\pm$0.005} \\
\modelname & $\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & \textbf{3.368$\pm$0.179} & \textbf{4.300$\pm$0.246} & \underline{0.325$\pm$0.014} & \textbf{0.411$\pm$0.016} & \underline{0.226$\pm$0.015} & \textbf{0.915$\pm$ 0.005} %l2: 0.23751, 0.008
  \\ \bottomrule
% COOKIE & SAT + POI + AOI + BF\textcolor{red}{DYNAMIC} & 3.6742$\pm$0.218 & 4.616$\pm$0.3 & 0.216$\pm$0.01 & 107.367$\pm$3.803 & 161.397$\pm$12.609 & 0.305$\pm$0.035
%   \\ \bottomrule
% COOKIE & SAT + POI + AOI + (BF)\textcolor{red}{concat bf} & 3.443$\pm$0.177 & 4.398$\pm$0.262 & 0.297$\pm$0.021 & 101.929$\pm$2.649 & 147.535$\pm$13.45 &0.357$\pm$0.029
  % \\ \bottomrule
\end{tabular}
\label{table_result_2}
\end{adjustbox}
\end{table*}



% \subsection{Population Density Prediction}
% Our contribution: unique info + shared info in fusion
% light-weight version of FactorCL => less complicated 

% MGFN: one modality, intra- and inter-view learning
% MVURE: multiple modalities, simple concat
% RegionDCL: dual contrastive learning: group-level, region-level (inter-region) correlation
% Urban2Vec: two modals with triplet loss
% KnowCL: inter-view contrastive learning between kg and mob
% FactorCL: heavy version, high dimension, many optimization goals

%  inter only: mvure, knowcl
%  both: all the rest.

\subsection{Overall performance}
\subsubsection{Population density.}
Table~\ref{table_result_1} presents the performance on population density prediction. \modelname $(\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A})$ achieves a significant improvement of $\geq$8.1\% in $R^2$ compared to baselines. 
Specifically, \modelname ($\mathcal{B} + \mathcal{P} + \mathcal{A}$) shows an 8.5\% improvement compared to the models using $\mathcal{M}$, i.e., MGFN and MVURE. \modelname ($\mathcal{B} + \mathcal{P} + \mathcal{A}$) also outperforms the models using inter-view only, with a 28.5\% improvement over KnowCL and 4\% over FactorCL, indicating the importance of including intra-view learning. 

% Comparison with mobility-based models such as MGFN and MVURE, \modelname shows an 8.5\% improvement with $\mathcal{B} + \mathcal{P} + \mathcal{A}$. It is important to note that while MGFN and MVURE depend on human mobility data, \modelname achieves superior results without relying on the mobility data. 
% % compared to MVURE, which graph attention network for modality fusion and 29.9\% improvement with MGFN, which uses attention-based fusion.
% With the comparison with inter-view only models, \modelname significantly outperforms KnowCL with an improvement of 28. 5\% and 4\% improvement with FactorCL. These results indicate the importance of including intra-view learning.
% % Compared to inter-view only models, MVURE and KnowCL, \modelname consistently delivers better results. Specifically, \modelname shows an improvement of $\geq$8.2\% in $R^2$ with MVURE, an improvement of 28. 5\% in $R^2$ using KnowCL. With generalized FactorCL, \modelname shows 4\% improvement. These results indicate that including both intra- and inter-view learning leads to better performance. 

Furthermore, \modelname $(\mathcal{S} + \mathcal{P} + \mathcal{A})$ and \modelname $(\mathcal{B} + \mathcal{P} + \mathcal{A})$ achieve 1.6\% and 5.9\% improvements over models using spatial proximity, i.e., Urban2Vec and RegionDCL, respectively. 
% For intra- and inter-view learning models, \modelname using $\mathcal{S} + \mathcal{P} + \mathcal{A}$ and $\mathcal{B} + \mathcal{P} + \mathcal{A}$ outperform Urban2Vec and RegionDCL, showing improvements of 1.6\% and 5.9\%, respectively. 
% A comparison with Urban2Vec and RegionDCL which incorporates geographic proximity compared to \modelnamex, \modelname outperforms with an improvement of 5.9\% with RegionDCL and 1.6\% improvement in Urban2Vec. 
\begin{figure}[h]
    \centering
\includegraphics[width=0.4\textwidth]{figures/nyc_pop_semi.png}
    % \vspace{0.5em}
    \caption{Measuring spatial autocorrelation using Semivariogram plot for population density in NYC. X-axis represents the lag distance between regions, and Y-axis shows semivariance. Blue points indicate observed semivariance values, red bars reflect the number of region pairs per lag distance, and the green line represents the fitted Matheron model.}
    \label{fig:nyc_semivariogram}
\end{figure}
Figure~\ref{fig:nyc_semivariogram} illustrates the spatial autocorrelation of population density in NYC. The semivariogram uses Matheron estimator, which calculates the average squared difference between population density values at paired locations~\cite{oliver2015basic}.
The semivariogram reveals strong autocorrelation at short distances, where population values are highly similar within nearby regions. 
However, the flattening of the curve beyond a lag distance of $0.1$ indicates that spatial proximity becomes less useful for predicting population density as the distance between regions increases. 
The red bars show that many region pairs fall beyond this threshold, suggesting low spatial autocorrelation. This supports the claim that models like \modelnamex, which do not rely on spatial proximity, are effective for population prediction tasks.
Overall, capturing both shared and unique information through pairwise inter-view learning effectively learns region representations.
% The red bars, which represent the number of region pairs at lag distances, show that many pairs fall beyond the $0.1$ threshold, suggesting low spatial autocorrelation at these distances. This supports the claim that models not relying on spatial proximity, such as \modelnamex, are effective for population prediction tasks, as demonstrated by the large number of region pairs with minimal spatial dependency beyond this threshold.
% Therefore, leveraging spatial proximity will largely help ... %The flattening of the curve suggests that this spatial dependence diminishes beyond the flattened range.

% Despite models like Urban2Vec and RegionDCL leveraging intra- and inter-view learning with spatial proximity, \modelname, utilizing $\mathcal{S} + \mathcal{P} + \mathcal{A}$ and $\mathcal{B} + \mathcal{P} + \mathcal{A}$ outperform a 1.6\% and 5.9\%, respectively. 
% Overall, capturing both shared and unique information through pairwise inter-view learning effectively learns region representations. %, providing a comprehensive understanding of the regions.
% It is noteworthy that Urban2Vec and RegionDCL incorporate geographic proximity to structure positive and negative pairs in geographic-information-based contrastive learning frameworks.
% This is further supported by high spatial autocorrelation in population density in ground truth. 
% \begin{figure}[h]
%     \centering
% \includegraphics[width=0.48\textwidth]{figures/nyc_c_p.png}
%     % \vspace{0.5em}
%     \caption{Population and crime ground truth semivariogram plots in NYC}
%     \label{fig:nyc_semivariogram}
% \end{figure}
% Figure~\ref{fig:nyc_semivariogram} visualizes spatial autocorrelation in the population density and crime rate in New York City (NYC) using semivariogram analysis. 
% The analysis shows that both population density and crime rate have strong spatial autocorrelation at short distances, as indicated by the rapid increase in semivariant that levels off around 0.1 degrees in EPSG:4326. The semivariogram for population density suggests a high similarity of population values within nearby neighborhood areas. 
% For the comparison with the model learning intra- and inter-view learning, \modelname significantly outperforms with a 44\% improvement. This result demonstrates capturing unique information along with share information is beneficial. 
% ReMVC, which utilizes contrastive learning in intra- and inter-view learning, our approach significantly outperforms with a 44\% improvement. These results highlight \modelname's effectiveness in not only capturing shared information across modalities but also preserving modality-specific features.

%  inter only: mvure, knowcl
%  both: all the rest.

\subsubsection{Crime rate.}
Table~\ref{table_result_1} shows that \modelname $(\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A})$ significantly outperforms all baselines with a $\geq$4.9\% improvement in $R^2$.
\modelname $(\mathcal{S} + \mathcal{P} + \mathcal{A})$ achieves a 5.6\% improvement over RegionDCL and only 0.4\% worse than Urban2Vec when using the same modalities.
\begin{figure}[h]
    \centering
\includegraphics[width=0.4\textwidth]{figures/nyc_crime_semi.png}
    % \vspace{0.5em}
    \caption{Semivariogram of crime rate in NYC.}
    \label{fig:nyc_semivariogram_crime}
\end{figure}
In particular, Figure~\ref{fig:nyc_semivariogram_crime} shows the spatial autocorrelation of crime rates in NYC. The spatial autocorrelation pattern is similar to population density, with a strong correlation at short distances but flattening beyond a lag of nearly $0.05$. The rise in red bars on the flattened part of the plot indicates many region pairs lack strong spatial autocorrelation, which indicates models like \modelname that do not rely on proximity are more suitable for predicting crime than the models using spatial information in their learning objectives (i.e., RegionDCL and Urban2Vec).
% Figure~\ref{fig:nyc_semivariogram_crime} presents the semivariogram of crime rates in NYC. Figure~\ref{fig:nyc_semivariogram_crime} shows a sharp increase in semivariance between 0.0 and 0.1 degree distance, which suggests that nearby neighboring regions tend to have similar crime rates. As the lag distance increases, the semivariance flattens, indicating that spatial correlation weakens as regions become further apart. 
% Despite this spatial pattern, \modelname excels without explicitly leveraging spatial information in the learning objectives, unlike Urban2Vec and RegionDCL.
In addition, \modelname ($\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$) outperforms MVURE and FactorCL by 6.8\% and 4\% in $R^2$, respectively, and achieves comparable results with KnowCL. This underscores the importance of intra-view learning in effectively capturing modality-specific information.
% that enhances overall \modelname performance.

% Urban2Vec uses geographic proximity for contrastive learning, while RegionDCL applies region-wise geographic information. Despite their use of spatial information in learning objectives, \modelname achieves comparable results to Urban2Vec without explicitly incorporating geographic information and surpasses RegionDCL's performance.

% Given the strong spatial autocorrelation in crime rates, Urban2Vec uses geographic proximity information when generating positive and negative pairs for inter-view contrastive learning, while RegionDCL utilizes region-wise contrastive learning based on geographic information. 
% Despite Urban2Vec and RegionDCL's advantage in utilizing spatial information, \modelname achieves comparable performance to Urban2Vec without explicitly relying on geographic information and surpasses RegionDCL's performance.

% This may be due to the high spatial autocorrelation observed in crime rates, which Urban2Vec’s triplet loss effectively leverages by capitalizing on the spatial relationships among regions.
% As indicated in Figure~\ref{fig:nyc_semivariogram}, the semivariogram for the crime rate demonstrates a strong spatial autocorrelation at short distances, which means that crime rates are likely to be similar to nearby neighborhoods.
% wever, \modelname still achieves improved performance without relying on the geographic adjacency information used in RegionDCL and Urban2Vec. 

%as indicated by Moran's I of 0.419 for the task. Although spatial autocorrelation is weaker than population density, it exists in crime rate as shown by Geary's C of 0.59832, which indicates less dissimilarity between neighboring regions.
% However, \modelname still achieves improved performance without relying on the geographic adjacency information used in RegionDCL and Urban2Vec. 

% However, our model still achieves improved performance without relying on the geographic adjacency information used in RegionDCL and Urban2Vec. Additionally, \modelname surpasses baselines utilizing $\mathcal{B} + \mathcal{P} + \mathcal{A}$, $\mathcal{B} + \mathcal{P} + \mathcal{M}$, or $\mathcal{M}$, demonstrating our model's effectiveness in capturing both unique and shared task-relevant information in multi-modal learning.

\subsubsection{Greenness.}
Table~\ref{table_result_2} presents greenness prediction in \textbf{NYC}. \modelname $(\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A})$ outperforms most baseline methods with $\geq$3.5\% in $R^2$ compared to RegionDCL, FactorCL, and MVURE, and similar performance to Urban2Vec with 1.2\% difference in $R^2$.
% outperforms most baseline methods and achieves performance comparable to intra- and inter-view models incorporating geographic information, Urban2Vec and RegionDCL. 
% Compared with the inter-view-only model, \modelname with $\mathcal{B} + \mathcal{P} + \mathcal{A}$ outperforms MVURE by 10.9\% and FactorCL by 3.2\% in $R^2$. But, Urban2Vec outperforms \modelname with $\mathcal{S} + \mathcal{P} + \mathcal{A}$ by 8.6\% in $R^2$. 
Furthermore, Table~\ref{table_result_delhi} shows $R^2$ in predicting greenness in \textbf{Delhi}. \modelname ($\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ and $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$) significantly outperforms Urban2Vec and RegionDCL by 15.56\% and 3.4\%, respectively. 

The performance variation between NYC and Delhi may be due to differences in region sizes and their varying satellite imagery features. Small regions tend to contain a large number of black pixels in the background in order to resize for input consistency with large regions.
Figure~\ref{fig_result_gvi} compares the absolute error distribution for greenness prediction between Urban2Vec and \modelname ($\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$). 
In NYC, 34\% of regions (799 out of 2160) are smaller than the standard input satellite imagery size. Urban2Vec has 576 regions with an error above 0.83, the lowest error range, while \modelname reduces the regions to 570. The difference in error distribution in these small regions is shown in subplots 1,4 and 2,5 of Figure~\ref{fig_result_gvi}, where \modelname shows lighter shading that indicates a lower error distribution.
In Delhi, \modelname consistently shows a lighter error distribution across the city, as seen in subplots 3 and 6.
Among 62\% of small regions (157 out of 253), Urban2Vec shows 94 regions with an error above 0.027, while \modelname only has 79 regions. 
% The performance variation between NYC and Delhi may be due to differences in variation in satellite imagery. In particular, a large region contains the large number of black pixels due to match the regularity input size with the other regions. 
% % The performance variation between NYC and Delhi may be due to differences in urban morphology, which means Delhi's larger geographic size and different neighborhood layouts play key roles.
% Figure~\ref{fig_result_gvi} visualizes the absolute error distribution for greenness prediction, comparing Urban2Vec with \modelname ($\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$). In NYC, irregularly shaped neighborhoods highlighted by the yellow circles exhibit darker colors that indicate higher error rates in Urban2Vec.
% These areas, characterized by non-uniform, complex boundaries, deviate from typical four-sided block patterns. 
% In these challenging regions, \modelname exhibits lighter shading compared to Urban2Vec, indicating a lower error rate. This suggests that \modelnamex handles irregularly shaped neighborhoods more effectively, highlighting the importance of accounting for local spatial characteristics beyond geographic size.
% Meanwhile, in Delhi, \modelname demonstrates a consistently lighter error distribution, indicating a lower error rate throughout the city. This result highlights the robustness of \modelnamex, as it maintains consistent performance regardless of geographic boundary size or region variations across countries. 

% with 1.2\% difference. 
% Urban2Vec records the highest $R^2$ at 33.7\%, followed by \modelname at 31.3\% and RegionDCL at 29\%. 

\begin{figure}[h]
    \centering
\includegraphics[width=0.45\textwidth]{figures/error_fig_v2.png}
    % \vspace{0.5em}
    \caption{Absolute error in Greenness in NYC and Delhi between Urban2Vec and COOKIE with $\mathcal{S}+\mathcal{P}+\mathcal{A}$. The lighter the color (close to white), the smaller the absolute error.}
    \label{fig_result_gvi}
\end{figure}
    
% This performance difference may be due to the smaller geographic tract sizes in NYC, where nearby tracts influence each other strongly.  
% Figure~\ref{fig_result_gvi} illustrates the absolute error distribution in greenness prediction, with images 1, 3, and 5 generated by Urban2Vec and 2, 4, and 6 by \modelnamex. In densely populated areas with small tracts, Urban2Vec shows higher errors than \modelname.
% In a similar vein, we observe the overall error distribution in \textbf{Delhi} learned by Urban2Vec is higher than \modelname by comparing with images 5 and 6 in Figure~\ref{fig_result_gvi}. Table~\ref{table_result_delhi} shows quantitative results in predicting greenness performance, as \modelname significantly outperforms Urban2Vec and RegionDCL by 15.56\% and 3.4\%, respectively. 
% Interestingly, \modelname with $\mathcal{B} + \mathcal{P} + \mathcal{A}$ outperforms \modelname with $\mathcal{S} 
% + \mathcal{B} + \mathcal{P} + \mathcal{A}$. This may be due to the lower spatial resolution available in Delhi compared to the high spatial resolution in NYC.  

% \begin{figure}[h]
%     \centering
% \includegraphics[width=0.45\textwidth]{figures/gvi_horizontal.png}
%     % \vspace{0.5em}
%     \caption{Absolute error in Greenness in NYC and Delhi between Urban2Vec (1,3,5) and COOKIE with $\mathcal{S}+\mathcal{P}+\mathcal{A}$ (2,4,6). The lighter the color (close to white), the smaller the absolute error.}
%     \label{fig_result_gvi}
% \end{figure}
\vspace{-1em}
\begin{table}[h]
\centering
\caption{Compare \modelname to baselines on Greenness in Delhi.}
\begin{adjustbox}{width=0.8\columnwidth,center}
  \begin{tabular}{l | c | c} \toprule
  Methods & Modalities & Greenness ($R^2$) \\ \midrule
  Urban2Vec & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.1916$\pm$0.051\\
  RegionDCL & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.2725$\pm$0.152\\
  % COOKIE &$\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.3515$\pm$0.1037\\ 
  \modelname &$\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.318$\pm$0.088\\
  \modelname &$\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.3459$\pm$0.069\\
  \modelname &$\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.3198$\pm$0.082 \\ \bottomrule
  \end{tabular}
  \label{table_result_delhi}
  \end{adjustbox}
\end{table}



% \textbf{Delhi.} We evaluate \modelname on Delhi in Table~\ref{table_result_delhi}, where has larger ward boundary compared to NYC. In Table~\ref{table_result_delhi}, \modelname outperforms Urban2Vec and RegionDCL by 15.56\% and 3.4\%, respectively.
% Specifically, in Figure~\ref{}, 5 and 6 figures represent absolute error distribution in Delhi by learning Urban2Vec and \modelnamex. As we can see, image 5 include a wide distribution of redness than image 6. Additionally, we can check that each geographic partition is larger than partitions in NYC. Thus, geographic adjacency information might not strongly require in some location, like Delhi. 

% {\color{red}\textbf{Delhi.} We evaluate \modelname on Delhi in Table~\ref{table_result_delhi}, where has larger ward boundary compared to NYC.}
% % which has incomplete and sparse data and lower image resolution compared to NYC. 
% In Table~\ref{table_result_delhi}, \modelname outperforms Urban2Vec and RegionDCL by 15.56\% and 3.4\%, respectively, demonstrating \modelnamex's effectiveness in regions, where spatial autocorrlation is weak. 
% Interestingly, \modelname with $\mathcal{S} + \mathcal{P} + \mathcal{A}$ outperforms $\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A}$. This may be due to Delhi's sparse building distribution, building footprints are not as densely packed as in NYC. This sparsity makes it challenging for models to capture meaningful patterns from building shapes and arrangement. 


% urban2vec: bag-of-words and add fclass (textual information)- more informative
\subsubsection{Land Use Classification}
Table~\ref{table_result_2} shows that \modelname $(\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A})$ outperforms all baselines and \modelname ($\mathcal{S} + \mathcal{P} + \mathcal{A}$) and Urban2Vec perform similarly overall. 
% The comparable results may be because the land use ground truth is represented as evaluating a probability distribution across five classes per region (e.g., a region's vector might look like [0.001, 0.09, 0.8, 0.1, 0.009].) 
% In addition, Urban2Vec incorporates geographic information in its learning objectives and uses a non-categorized POI modality, unlike \modelnamex, allowing it to capture subtle distinctions across the five categories. 
The comparable results may be attributed to Urban2Vec utilizing fine-grained representations of $\mathcal{P}$ and $\mathcal{A}$, whereas \modelname employs these features in a categorized format.
While Urban2Vec benefits from the additional geographic information, \modelname achieves similar results without it. 
In comparison with FactorCL, which captures both shared and unique features in $\mathcal{B} + \mathcal{P} + \mathcal{A}$, \modelname outperforms 5.3 in L1, indicating the effectiveness of the pairwise inter-view learning approach.
% Table~\ref{table_result_2} shows that \modelname using $\mathcal{S} + \mathcal{B} + \mathcal{P} + \mathcal{A}$ outperforms all baselines by at least 1\% in $L1$ for land use classification. Methods that incorporate spatial proximity in their learning objectives, such as Urban2Vec and RegionDCL, achieve better results than others like MGFN and MVURE.
% When comparing \modelname ($\mathcal{S} + \mathcal{P} + \mathcal{A}$) with Urban2Vec, both show comparable overall performance. This may be because the land use ground truth is represented as a probability distribution across five classes per region, and Urban2Vec’s triplet loss, which leverages spatial relationships and uses fine-grained POI counts instead of predefined categories, can effectively capture these subtle variations.
% While Urban2Vec benefits from the additional geographic information, \modelname achieves similar results without it.
% In comparison with FactorCL, \modelname shows superior overall performance, which indicates the effectiveness of the pairwise inter-view learning approach.

\subsection{Ablation Study}
% \subsubsection{Without Intra-view \& $U$ in Inter-view}
\subsubsection{Ablations on Learning Objectives}
We conduct ablation studies by removing intra-view learning (\modelname-IR) and unique feature extraction in inter-view learning (\modelname-UR) 
% (\modelname-UniqueRemoved) 
from \modelname to evaluate the contribution of each component. Table~\ref{table_result_ablation} reports the $R^2$ results for two downstream tasks, greenness and crime rate, which reflect the regions' public health and socioeconomic conditions. As shown, \modelname consistently outperforms both variants on the two tasks.

For greenness prediction, \modelname-UR shows a significant performance drop of 8.4\% compared to \modelnamex. This result aligns with our expectation, as greenness is closely tied to $\mathcal{S}$, where visual features of greenery play a crucial role in predicting greenness.
In the crime rate prediction, \modelname outperforms both ablated variants. Specifically, \modelname-UR shows a 6.9\% reduction in performance compared to \modelnamex, demonstrating the importance of unique feature extraction for crime rate prediction. 
Given that crime rates are influenced by various socioeconomic and spatial factors, such as proximity to police stations or activity on main streets, \modelnamex’s ability to capture unique features across modalities leads to comprehensive representation.
Additionally, comparing \modelname-IR to \modelnamex, we observe a reduction of 2.4\% in crime prediction. This result indicates that intra-view learning, which focuses on capturing modal-specific information by comparing other regions, contributes to learning complementary details within each modality. 
% We remove intra-view learning (\modelname - no intra) and unique features in inter-view learning (\modelname - no unique) from \modelname to demonstrate each component's effectiveness. 
% Table~\ref{table_result_ablation} presents the $R^2$ results for two downstream tasks, greenness and crime rate, which reflect the regions' public health and socioeconomic conditions. As shown in Table~\ref{table_result_ablation}, \modelname outperforms its variants \modelname - no intra and \modelname - no unique across both tasks. 
% % representing regions' public health and socioeconomic aspects. \modelname outperforms its variants \modelname - no intra and \modelname - no unique across both tasks. 
% Notably, predicting greenness using \modelname - no unique shows downgraded performance than \modelnamex by a 8.4\%. This result is aligned with intuition where greenness is visible through $\mathcal{S}$, which demonstrates the effectiveness of high unique features in $\mathcal{S}$. 
% % These findings indicate that both objectives are essential for the overall effectiveness of our model.
\begin{table}[htbp]
\centering
\caption{Ablation study on Greenness and Crime ($R^2$) in NYC.}
\begin{adjustbox}{width=0.85\columnwidth,center}
  \begin{tabular}{l | c | c | c}  \toprule
  Methods & Modalities & Greenness & Crime \\ \midrule
  \multirow{3}{*}{\modelname-IR} & $\mathcal{S}$ + $\mathcal{P}$ + 
   $\mathcal{A}$ &  0.234$\pm$0.035 & 0.275$\pm$0.029 \\
   & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.259$\pm$0.015 & 0.336$\pm$0.039 \\\midrule
   \multirow{3}{*}{\modelname-UR}& $\mathcal{S}$ + $\mathcal{P}$ + 
   $\mathcal{A}$ & 0.166$\pm$0.024 & 0.26$\pm$0.0293 \\
   & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.285$\pm$0.015 & 0.322$\pm$0.03 \\ \midrule
  \multirow{3}{*}{\modelname} & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.25$\pm$0.07 & 0.322$\pm$0.03 \\
  & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.292$\pm$0.01 & 0.346$\pm$0.017 \\
   \bottomrule
  \end{tabular}
  \label{table_result_ablation}
\end{adjustbox}
\end{table}


% \begin{table}[htbp]
% \centering
% \caption{Ablation study on Population and Crime ($R^2$) in NYC.}
% \begin{adjustbox}{width=1.0\columnwidth,center}
%   \begin{tabular}{l | c | c | c}  \toprule
%   Methods & Modalities & Population & Crime \\ \midrule
%   \multirow{3}{*}{\modelname - no intra} & $\mathcal{S}$ + $\mathcal{P}$ + 
%    $\mathcal{A}$ & 0.6 $\pm$ 0.022& 0.275$\pm$0.029 \\
%    & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.611$\pm$0.017 & 0.336$\pm$0.039 \\\midrule
%    % &$\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.695$\pm$0.019 & 0.375$\pm$0.039 \\ \midrule
%    \multirow{3}{*}{\modelname - no unique}& $\mathcal{S}$ + $\mathcal{P}$ + 
%    $\mathcal{A}$ & 0.50$\pm$0.014 & 0.26$\pm$0.0293 \\
%    & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$& 0.65$\pm$0.017 & 0.322$\pm$0.03 \\ \midrule
%   \multirow{3}{*}{\modelname} & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.63$\pm$0.033 & 0.322$\pm$0.03 \\
%   & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.627$\pm$0.009 & 0.346$\pm$0.017 \\
%    % &$\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 0.698$\pm$0.017 & 0.377$\pm$0.017 \\ 
%    \bottomrule
%   \end{tabular}
%   \label{table_result_ablation}
% \end{adjustbox}
% \end{table}

\subsubsection{Effect of Modalities}
Figure~\ref{all_2} illustrates the impact of using different modalities on the performance of FactorCL and \modelnamex. 
The results reveal a consistent pattern: adding $\mathcal{S}$ and $\mathcal{B}$ significantly boosts performance across most tasks. \modelname with $\mathcal{S} + \mathcal{B}+ \mathcal{P}+ \mathcal{A}$ consistently outperform \modelname with three modals combinations across all four tasks. 
In comparison, FactorCL using two modalities shows weaker performance overall. This suggests that using fewer modalities limits the model's ability to capture the full complexity of region features, as it lacks the rich information provided by the additional modalities.
The contrast between FactorCL and \modelname shows the importance of using multiple modalities rather than relying on modality pairs in region representation learning to generate comprehensive representations.
% Although the AOI and SAT pair do not perform well in FactorCL across four tasks, \modelname effectively extracts task-relevant features, leading to improved results.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/all_mm_v2.png}
    \vspace{0.5em}
    % \caption{Effect of Modalities. We show $R^2$ on population, greenness, and crime, and $L1$ on land use task.}
    \caption{Effect of Modalities. We show $R^2$ on population density, greenness, and crime rate, and $L1$ on land use task.}
    \label{all_2}
\end{figure}

% \begin{figure}
% \vspace{-0.8em}
% \setlength{\belowcaptionskip}{-9pt}
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/all.png}
%         \caption{Single modal testing}
%         % \vspace{-2em}
%         \label{all_single}
%     \end{subfigure}
%     % \vspace{2em}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/all_mm.png}
%         \caption{Multi modal testing}
%         \label{all_multi}
%         % \vspace{-2em}
%     \end{subfigure}
%     \vspace{2em}
%     \caption{Modality Performance Testing}
%     \label{all_testing}
%     \hfill
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/all.png}
%     \vspace{0.5em}
%     \caption{Single modal testing}
%     \label{all_1}
% \end{figure}




% \begin{table*}[htbp]
% \centering
% \caption{Tabel1-1: Compare COOKIE to existing SOTA approaches on tasks in NYC. }
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Population}} & \multicolumn{3}{c}{\textbf{Land Use}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {L1}$\downarrow$ & {KL}$\downarrow$ & {Cosine}$\uparrow$\\
% \midrule
% RegionDCL & BF + POI & 5020.20$\pm$216.63 & 6960.51$\pm$282.35 & 0.575$\pm$0.039 & \underline{0.418$\pm$0.010} & \underline{0.229$\pm$0.008} & \underline{0.912$\pm$0.004}  \\
% Urban2Vec & SAT + POI & 5328.38$\pm$200.58  & 7410.42$\pm$261.89  & 0.522$\pm$0.028 & 0.473$\pm$0.018 & 0.295$\pm$0.015 & 0.890$\pm$0.007 \\
% MVURE & MOB + POI & 6557.12$\pm$265.30 & 8307.58$\pm$329.44 & 0.404$\pm$0.034 & 0.542$\pm$0.014 & 0.329$\pm$0.014 & 0.872$\pm$0.006  \\
% MGFN & MOB & 6754.579$\pm$201.134 & 8989.136$\pm$312.712 & 0.331$\pm$0.05 & 0.53$\pm$0.012 & 0.334$\pm$0.011 & 0.875$\pm$0.006  \\
% KnowCL & SAT + KG &00 & 00 & 00 & 00 & 00 & 00  \\ \midrule
% % WWW~\cite{xi2022beyond} & SAT + POI & 00 & 00 & 00 & 00 & 00 & 00  \\ 
% % WWW23~\cite{www23} & 4 (MOB+POI+LOC+BUS) KG & 3981.866$\pm$170.111 & 5532.106$\pm$295.059 & 0.706$\pm$0.03 & 0.401$\pm$0.008 & 0.211$\pm$0.01 & 0.921$\pm$0.003 \\\midrule
% COOKIE & SAT + POI + AOI  & \underline{4874.206$\pm$131.633} & \underline{6420.222$\pm$190.87} & \underline{0.6$\pm$0.022} & 0.455$\pm$0.009 & 0.250$\pm$0.009 & 0.906$\pm$0.004  \\ 
%  \midrule
% % COOKIE & SAT + POI + AOI + BF\textcolor{red}{STATIC} & \textbf{4359.089$\pm$128.836} & \textbf{5788.659$\pm$209.536} & \textbf{0.6624$\pm$0.013} & 0.6009$\pm$0.009 & 0.3821$\pm$0.005 & 0.8506$\pm$0.003
% %   \\ \bottomrule
%   COOKIE & SAT + POI + AOI + BF& \textbf{4096.229$\pm$159.038} & \textbf{5824.79$\pm$197.989} & \textbf{0.695$\pm$0.019} & \textbf{0.39$\pm$0.016} & \textbf{0.203$\pm$0.011} & \textbf{0.923$\pm$0.005}
%   \\ \bottomrule
% % COOKIE & SAT + POI + AOI + (BF)\textcolor{red}{concat bf} & 4300.936$\pm$120.867 & 5926.12$\pm$157.301 & 0.675$\pm$0.017 &  
%   % \\ \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{Compare COOKIE to existing SOTA approaches on tasks in NYC. $\downarrow$ means the smaller value is the better, while $\uparrow$ means the larger value is the better. We highlight the best result as the bold and the runner-up performance as the underline. }
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Population}} & \multicolumn{3}{c}{\textbf{Crime}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$\\
% \midrule
% Urban2Vec & SAT + POI & 5328.38$\pm$200.58  & 7410.42$\pm$261.89  & 0.522$\pm$0.028 & 124.432$\pm$5.168 & 185.318$\pm$14.252 & 0.151$\pm$0.058 \\
% MVURE & MOB + POI & 6557.12$\pm$265.30 & 8307.58$\pm$329.44 & 0.404$\pm$0.034 & 114.548$\pm$2.545 & 161.039$\pm$10.128 & 0.242$\pm$0.035  \\
% MGFN & MOB & 6754.58$\pm$201.13 & 8989.14$\pm$312.71 & 0.331$\pm$0.05 & 116.089$\pm$4.407 & 161.942$\pm$9.862 & 0.231$\pm$0.043   \\
% KnowCL (log) & SAT + KG & - & 0.612 & 0.153 & - & 0.622 & 0.536  \\ 
% RegionDCL & BF + POI & 5020.20$\pm$216.63 & 6960.51$\pm$282.35 & 0.575$\pm$0.04 & 115.206$\pm$1.22 & 176.006$\pm$11.808 & 0.177$\pm$0.022  \\\midrule
% MVURE & MOB + BF + POI & 5295.00$\pm$101.72 & 7065.08$\pm$122.913 & 0.545$\pm$0.014 & 108.604$\pm$5.019 & 151.879$\pm$13.46 & 0.278$\pm$0.043 \\ 
% RegionDCL\color{red}{Yijun} & BF + POI + AOI & 4891.96$\pm$103.11 & 6890.84$\pm$164.84 & 0.568$\pm$0.013     & 106.00$\pm$2.36 & 163.71$\pm$15.17 & 0.290$\pm$0.0340  \\
% Urban2Vec\color{red}{Yijun} & SAT+ POI + AOI & 4760.066$\pm$191.453 & 6497.809$\pm$395.89 & 6497.809$\pm$395.89 & 104.95$\pm$3.499 & 159.289$\pm$12.241 & 0.326$\pm$0.04 \\ \midrule  \midrule 
% COOKIE & SAT + POI + AOI  & \underline{4874.206$\pm$131.633} & \underline{6420.222$\pm$190.87} & \underline{0.6$\pm$0.022} & \underline{111.904$\pm$2.883} & \underline{165.153$\pm$12.365} & \underline{0.275$\pm$0.029}  \\ 
% % COOKIE & BF + POI + AOI & 4691.688$\pm$68.933 & 6497.817$\pm$139.128 & 0.611$\pm$0.017 & \underline{102.313$\pm$4.563} & \underline{146.337$\pm$14.052} & \underline{0.336$\pm$0.036}  \\
% COOKIE & SAT + POI + AOI + BF& \textbf{4096.229$\pm$159.038} & \textbf{5824.79$\pm$197.989} & \textbf{0.695$\pm$0.019} & \textbf{98.92$\pm$2.3} & \textbf{145.352$\pm$14.35} & \textbf{0.375$\pm$0.039} \\ 
% COOKIE (log) & SAT + POI + AOI + BF  & - &  0.45 & 0.438 & - & 0.626 & 0.525 \\ \bottomrule
% % COOKIE & SAT + POI + AOI + (BF)\textcolor{red}{concat bf} & 4300.936$\pm$120.867 & 5926.12$\pm$157.301 & 0.675$\pm$0.017 &  
%   % \\ \bottomrule
% \end{tabular}
% \label{table_result_1}
% \end{table*}


% update version
% \begin{table*}[htbp]
% \centering
% \caption{Compare \modelname to baselines on population and crime prediction in NYC. $\downarrow$ means the smaller value is the better and $\uparrow$ is the opposite. We bold the best result and underscore the second best. The modalities used in the models include POIs ($\mathcal{P}$), AOIs ($\mathcal{A}$), satellite imagery ($\mathcal{S}$), building footprints ($\mathcal{B}$), and mobility ($\mathcal{M}$).}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Greenness}} & \multicolumn{3}{c}{\textbf{Land Use}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {L1}$\downarrow$ & {KL}$\downarrow$ & {Cosine}$\uparrow$\\
% \midrule
% MGFN & $\mathcal{M}$ & 3.949$\pm$0.187 & 5.032$\pm$0.255 & 0.094$\pm$0.023 & 0.53$\pm$0.012 & 0.334$\pm$0.011 & 0.875$\pm$0.006\\
% MVURE & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{M}$ & 3.723$\pm$0.201 & 4.875$\pm$0.259 & 0.183$\pm$0.039 & 0.526$\pm$0.008 & 0.337$\pm$0.011 & 0.872$\pm$0.006 \\ 
% % 
% Urban2Vec & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$& 3.373$\pm$0.163 & 4.423$\pm$0.239
%  & 0.337$\pm$0.028 & 0.422$\pm$0.017 & 0.241$\pm$0.019 & 0.91$\pm$0.006 \\\midrule \midrule   
% % 
% RegionDCL & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 3.481$\pm$0.176 & 4.574$\pm$0.254 & 0.29$\pm$0.032 & 0.412$\pm$0.012 & 0.241$\pm$0.02 & 0.911$\pm$0.006 \\ \midrule  \midrule 
% % 
% \modelname & $\mathcal{S}$ + $\mathcal{P}$ + $\mathcal{A}$  & 3.627$\pm$0.165 & 4.714$\pm$0.237 & 0.234$\pm$0.035 & 0.455$\pm$0.009 & 0.250$\pm$0.009 & 0.906$\pm$0.004  \\ 
% \modelname & $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & 3.53$\pm$0.174 & 4.49$\pm$0.267 & 0.259$\pm$0.015 &0.594$\pm$0.008 & 0.379$\pm$0.006 & 0.851$\pm$0.004 \\
% \modelname & $\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$ & \textbf{3.398$\pm$0.173} & \textbf{4.266$\pm$0.27} & \textbf{0.313$\pm$0.022} & \textbf{0.39$\pm$0.016} & \textbf{0.203$\pm$0.011} & \textbf{0.923$\pm$0.005} \midrule \midrule 
% KnowCL (log) & $\mathcal{S}$ + \textit{KG} & - & 0.612 & 0.153 & - & 0.622 & 0.536  \\ 
% \modelname (log) & $\mathcal{S}$ + $\mathcal{B}$ + $\mathcal{P}$ + $\mathcal{A}$  & - &  0.45 & 0.438 & - & 0.626 & 0.525 \\ \bottomrule
% \end{tabular}
% \label{table_result_2}
% \end{table*}


% \begin{table*}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Population}} & \multicolumn{3}{c}{\textbf{Crime}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$\\
% \midrule
% COOKIE & center &5287.638$\pm$223.051 & 7103.917$\pm$357.374& 0.5273$\pm$0.049 & 111.173$\pm$2.572 & 158.353$\pm$11.641 & 0.2818$\pm$0.015 \\
% COOKIE & tract &6260.903$\pm$24.756 & 8275.463$\pm$98.564& 0.38631$\pm$0.0179 & 120.5$\pm$3.59 & 168.29$\pm$12.425 & 0.19$\pm$0.033  \\ \midrule  \midrule 
% COOKIE & mosaic  & \underline{4874.206$\pm$131.633} & \underline{6420.222$\pm$190.87} & \underline{0.6$\pm$0.022} & \underline{111.904$\pm$2.883} & \underline{165.153$\pm$12.365} & \underline{0.275$\pm$0.029}  \\ \bottomrule
% \end{tabular}
% \label{table_result_ablation_1}
% \end{table*}

% \begin{table*}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Greenness}} & \multicolumn{3}{c}{\textbf{Land Use}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {L1}$\downarrow$ & {KL}$\downarrow$ & {Cosine}$\uparrow$\\
% \midrule
% COOKIE & center & 3.659$\pm$0.17 & 4.583$\pm$0.255 & 0.221$\pm$0.01 & 0.31$\pm$0.01 & 0.514$\pm$0.01 & 0.882$\pm$0.004\\
% COOKIE & tract & 3.917$\pm$0.206 & 4.96$\pm$0.27 & 0.118$\pm$0.018 & 0.381$\pm$0.005 & 0.596$\pm$0.006 & 0.851$\pm$0.004\\
% \midrule  \midrule 
% COOKIE & mosaic  & 3.627$\pm$0.165 & 4.714$\pm$0.237 & 0.234$\pm$0.035 & 0.455$\pm$0.009 & 0.250$\pm$0.009 & 0.906$\pm$0.004\\ \bottomrule
% \end{tabular}
% \label{table_result_ablation_2}
% \end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{Compare COOKIE to the baselines using three modalities}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Population}} & \multicolumn{3}{c}{\textbf{Land Use}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {L1}$\downarrow$ & {KL}$\downarrow$ & {Cosine}$\uparrow$\\
% \midrule
% MGFN & MOB & 6754.579$\pm$201.134 & 8989.136$\pm$312.712 & 0.331$\pm$0.05 & 0.53$\pm$0.012 & 0.334$\pm$0.011 & 0.875$\pm$0.006  \\
% MVURE & MOB + POI & 6557.12$\pm$265.30 & 8307.58$\pm$329.44 & 0.404$\pm$0.034 & 0.542$\pm$0.014 & 0.329$\pm$0.014 & 0.872$\pm$0.006\\
% MVURE & MOB + POI + BF & 5295.00$\pm$101.72 & 7065.08$\pm$122.913 & 0.545$\pm$0.014 & 0.526$\pm$0.008 & 0.337$\pm$0.011 & 0.872$\pm$0.006  \\ 
% RegionDCL & BF + POI & 5020.20$\pm$216.63 & 6960.51$\pm$282.35 & 0.575$\pm$0.039 & 0.418$\pm$0.010 & 0.229$\pm$0.008 & 0.912$\pm$0.004 \\ 
% RegionDCL & BF + POI + AOI & \\ \midrule
% COOKIE &  BF + POI + AOI &  4691.688$\pm$68.933 & 6497.817$\pm$139.128 & 0.611$\pm$0.017 & 0.594$\pm$0.008 & 0.379$\pm$0.006 & 0.851$\pm$0.004 \\ \midrule   
% Urban2Vec & SAT+ [POI + AOI] & \\ \midrule   
% COOKIE & SAT + POI + AOI & 4874.206$\pm$131.633 & 6420.222$\pm$190.87 & 0.6$\pm$0.022 & 0.455$\pm$0.009 & 0.250$\pm$0.009 & 0.906$\pm$0.004 \\   
%   COOKIE & SAT + POI + AOI + BF & 4096.229$\pm$159.038 & 5824.79$\pm$197.989 & 0.695$\pm$0.019 & 0.39$\pm$0.016 & 0.207$\pm$0.011 & 0.922$\pm$0.005 \\ \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{Compare COOKIE to the baselines using three modalities}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{GVI}} & \multicolumn{3}{c}{\textbf{Crime}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ &  {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ \\
% \midrule
% MGFN & MOB & 3.949$\pm$0.187 & 5.032$\pm$0.255 & 0.094$\pm$0.023 & 116.089$\pm$4.407 & 161.942$\pm$9.862 & 0.231$\pm$0.043  \\
% MVURE & MOB + POI & 4.067$\pm$0.272 & 5.186$\pm$0.338 & 0.048$\pm$0.029 & 114.548$\pm$2.545 & 161.039$\pm$10.128 & 0.242$\pm$0.035  \\
% MVURE & MOB + POI + BF & 3.723$\pm$0.201 & 4.875$\pm$0.259 & 0.183$\pm$0.039 & 108.604$\pm$5.019 & 151.879$\pm$13.46 & 0.278$\pm$0.043  \\ 
% RegionDCL & BF + POI & 3.433$\pm$0.198 & 4.547$\pm$0.298 & 0.298$\pm$0.03 & 115.206$\pm$1.217 & 176.006$\pm$11.808 & 0.177$\pm$0.022  \\ 
% RegionDCL & BF + POI + AOI & \\ \midrule
% COOKIE &  BF + POI + AOI & 3.53$\pm$0.174 & 4.49$\pm$0.267 & 0.259$\pm$0.015 & 102.313$\pm$4.563 & 146.337$\pm$14.052 & 0.336$\pm$0.036 \\ \midrule \midrule  
% Urban2Vec & SAT+ [POI + AOI] & \\ \midrule   
% COOKIE & SAT + POI + AOI & 3.627$\pm$0.165 & 4.714$\pm$0.237 & 0.234$\pm$0.035 & 111.904$\pm$2.883 & 165.153$\pm$12.365 & 0.275$\pm$0.029 \\   
%   COOKIE & SAT + POI + AOI + BF & \textbf{3.398$\pm$0.173} & \textbf{4.266$\pm$0.27} & \textbf{0.313$\pm$0.022} & \textbf{98.92$\pm$2.3} & \textbf{145.352$\pm$14.35} & \textbf{0.375$\pm$0.039} \\ \bottomrule
% \end{tabular}
% \end{table*}



% \begin{figure}[h]
% % \vspace{-0.8em}
% \setlength{\belowcaptionskip}{-9pt}
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/R2_pop.png}
%         \caption{Population Density}
%         \label{r2_pop}
%     \end{subfigure}
%     \vspace{2em}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/R2_Crime.png}
%         \caption{Crime}
%         \label{r2_crime}
%     \end{subfigure}\\
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/R2_Greenness.png}
%         \caption{Greenness}
%         \label{r2_green}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Cosine_Land_Use.png}
%         \caption{Land Use}
%         \label{cos_land}
%     \end{subfigure}\\
%     \hfill
%     \caption{Robustness Testing on NYC}
%     \label{modal_testing}
% \end{figure}



% \begin{table*}[htbp]
% \centering
% \caption{temporary, will turn into figures}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Population}} & \multicolumn{3}{c}{\textbf{Land Use}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {L1}$\downarrow$ & {KL}$\downarrow$ & {Cosine}$\uparrow$\\
% \midrule
%     RF & POI &  7128.773$\pm$150.815 & 9290.936$\pm$185.129 & 0.215$\pm$0.026 & 0.504$\pm$0.016 & 0.292$\pm$0.021 & 0.888$\pm$0.009 \\
%     RF & AOI & \underline{4635.876$\pm$289.236} & 6438.594$\pm$413.693 & \underline{0.623$\pm$0.048} & 0.45$\pm$0.016 & 0.244$\pm$0.011 & 0.912$\pm$0.009 \\
%     ResNet + RF & SAT & 7225.861$\pm$216.684 & 9200.455$\pm$363.808 & 0.236$\pm$0.055 & \textbf{0.374$\pm$0.009} & \textbf{0.185$\pm$0.004} & \underline{0.92$\pm$0.003}  \\
%     ResNet + RF & BF & 6635.81$\pm$308.903 & 8717.787$\pm$398.56 & 0.307$\pm$0.047 & 0.508$\pm$0.007 & 0.306$\pm$0.007 & 0.882$\pm$0.003 \\  \midrule
%     FactorCL & POI + AOI & 5189.736$\pm$148.635 & 7068.895$\pm$236.746 & 0.547$\pm$0.027 &  0.453$\pm$0.0109 & 0.252$\pm$0.012 & 0.905$\pm$0.006 \\
%     % FactorCL & AOI + SAT & 5377.826$\pm$334.312 & 7613.545$\pm$456.243 & 0.507$\pm$0.0561 & 0.6$\pm$0.008 & 0.382$\pm$0.005 & 0.85$\pm$0.004  \\  \midrule
%     FactorCL & AOI + SAT & 5438.917$\pm$270.061 & 7314.093$\pm$333.302 & 0.509$\pm$0.048 & 0.493$\pm$0.013 & 0.281$\pm$0.01 & 0.891$\pm$0.006  \\  \midrule
%     COOKIE & SAT + POI + AOI & 4874.206$\pm$131.633 & \underline{6420.222$\pm$190.87} & 0.6$\pm$0.022 & 0.455$\pm$0.009 & 0.250$\pm$0.009 & 0.906$\pm$0.004  \\ 
%     COOKIE & BF + POI + AOI & 4691.688$\pm$68.933 & 6497.817$\pm$139.128 & 0.611$\pm$0.017 & 0.594$\pm$0.008 & 0.379$\pm$0.006 & 0.851$\pm$0.004 \\ \midrule
%     % COOKIE & BF + POI + AOI\textcolor{red}{opt landuse}  & 5133.596$\pm$98.504 & 6993.844$\pm$144.59 & 0.534$\pm$0.023 & 0.506$\pm$0.01 & 0.313$\pm$0.009 & 0.878$\pm$0.004 \\ \midrule
%     COOKIE & SAT + POI + AOI + BF & \textbf{4096.229$\pm$159.038} & \textbf{5824.79$\pm$197.989} & \textbf{0.695$\pm$0.019} & \underline{0.39$\pm$0.016} & \underline{0.207$\pm$0.011} & \textbf{0.922$\pm$0.005}
%   \\ \bottomrule
%   % COOKIE & SAT + POI + AOI + BF\textcolor{red}{DYNAMIC} & 4683.227$\pm$142.74 & 6416.838$\pm$285.889 & 0.619$\pm$0.031 & 0.604$\pm$0.012 & 0.383$\pm$0.004 & 0.85$\pm$0.003
%   % \\ \bottomrule
% \end{tabular}
% \label{table: res4_1}
% \end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{temporary, will turn into figures}
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Greenness}} & \multicolumn{3}{c}{\textbf{Crime}}\\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} 
% \textbf{Methods} & \textbf{Modalities} & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$ & {MAE}$\downarrow$ & {RMSE}$\downarrow$ & {R2}$\uparrow$\\
% \midrule
%     RF & POI & 3.986$\pm$0.19 & 5.173$\pm$0.262 & 0.093$\pm$0.018 & 117.681$\pm$3.431 & 173.257$\pm$12.078 & 0.201$\pm$0.032 \\
%     RF & AOI & 3.6443$\pm$0.1928 & \underline{4.297$\pm$0.234} & 0.22$\pm$0.028 & 106.581$\pm$4.307 & 161.866$\pm$12.063 & 0.303$\pm$0.029 \\
%     ResNet + RF  & SAT & \underline{3.492$\pm$0.197} & 4.537$\pm$0.256 & \underline{0.303$\pm$0.016} & 130.314$\pm$9.15 & 188.256$\pm$18.657 & 0.069$\pm$0.052  \\
%     ResNet + RF & BF & 3.57$\pm$0.21 & 4.731$\pm$0.274 & 0.242$\pm$0.025 & 129.913$\pm$3.4 & 188.807$\pm$14.427 & 0.044$\pm$0.05  \\  \midrule
%     FactorCL & POI + AOI & 3.827$\pm$0.165 & 4.9$\pm$0.236 & 0.143$\pm$0.019 & 109.945$\pm$3.918 & 163.958$\pm$13.092 & 0.279$\pm$0.043\\
%     FactorCL & AOI + SAT & 3.708$\pm$0.207 & 4.814$\pm$0.262 & 0.194$\pm$0.028 & 126.097$\pm$3.897 & 177.819$\pm$13.268 & 0.123$\pm$0.038 \\  \midrule
%     COOKIE & SAT + POI + AOI  & 3.631$\pm$0.177 & 4.76$\pm$0.25 & 0.232$\pm$0.036 & 111.904$\pm$2.883 & 165.153$\pm$12.365 & 0.275$\pm$0.029  \\ 
%     COOKIE & BF + POI + AOI & 3.53$\pm$0.174 & 4.49$\pm$0.267 & 0.259$\pm$0.015 & \underline{102.313$\pm$4.563} & \underline{146.337$\pm$14.052} & \underline{0.336$\pm$0.036} \\ \midrule
%     % COOKIE & BF + POI + AOI\textcolor{red}{opt landuse} & 3.672$\pm$0.234 & 4.544$\pm$0.298 & 0.213$\pm$0.027 & 107.899$\pm$2.528 & 150.889$\pm$13.764 & 0.288$\pm$0.039 \\ \midrule
%     COOKIE & SAT + POI + AOI + BF & \textbf{3.398$\pm$0.173} & \textbf{4.266$\pm$0.27} & \textbf{0.313$\pm$0.022} & \textbf{98.92$\pm$2.3} & \textbf{145.352$\pm$14.35} & \textbf{0.375$\pm$0.039}
%   % COOKIE & SAT + POI + AOI + BF\textcolor{red}{DYNAMIC} & 3.674$\pm$0.218 & 4.616$\pm$0.3 & 0.216$\pm$0.01 & 107.367$\pm$3.803 & 161.397$\pm$12.609 & 0.305$\pm$0.035
%   \\ \bottomrule
% \end{tabular}
% \label{table: res4_2}
% \end{table*}


==> sections/_introduction.tex <==
\section{Introduction} 
In the past decade, the global urban population has grown rapidly from 52\% to 57\%~\cite{UNpop}, highlighting the need for effective urban planning and monitoring.
Socioeconomic indicators, such as population density, crime rate, and education level, serve as proxies to understand social and economic dynamics, aiding urban planning decisions that improve quality of life, public health, and community well-being. 
Traditional door-to-door demographic surveys conducted by the US Census Bureau provide detailed statistics but are labor intensive, time consuming, and costly, resulting in infrequent monitoring of cities~\cite{gebru2017using}. 


% With the increasing availability of data online, researchers have studied region representation learning (RRL), which provides a scalable alternative by leveraging various geospatial data such as remote sensing, street view imagery, and Point of Interest (POI) to predict socioeconomic indicators~\cite{jenkins2019unsupervised,yao2018representing,wang2017region,mvure,liu2023knowledge,li2022predicting}. 
Region representation learning (RRL) provides a scalable alternative by leveraging various geospatial data such as remote sensing, street view imagery, and Point of Interest (POI) to predict socioeconomic indicators~\cite{jenkins2019unsupervised,yao2018representing,wang2017region,mvure,liu2023knowledge,li2022predicting}. 
The goal of RRL is to learn a mapping function from multimodal geospatial data into a region representation by capturing relationships across data (modalities) and between regions.
Existing RRL studies often use contrastive learning to model these relationships effectively through intra-view and inter-view learning. Specifically, intra-view learning learns representations to be distinctive between regions within a single modality and inter-view learning aligns information from multiple modalities for a region. However, most contrastive learning-based RRL approaches~\cite{tkde,li2024urban} handle only two modalities or require specific data sources (e.g., human mobility), which limits their generalizability in adapting diverse geospatial data.

% Existing RRL studies often use multi-view contrastive learning, leveraging both intra-view and inter-view learning~\cite{tkde,li2024urban}. The intra-view learning aims to capture each view’s (modality’s) representation by maximizing discrepancy between regions within view, and the inter-view learning is to learn relationships across views. However, these approaches typically utilize two modalities (e.g., Points of Interest and human mobility), constraining the model’s capacity and limiting its applicability in regions where mobility data are not universally available. 

% {\color{purple} Recently, multimodal representation learning has achieved great success in computer vision and natural language processing domains by aligning more than three modalities~\cite{imagebind,zhu2023languagebind}. However, these approaches generally learn the mutual information $I(x1; x2)$ (where $x1$ and $x2$ are modalities) between modalities without considering any conditional information, thereby overlooking unique information during inter-view contrastive learning. }

Existing work in computer vision and natural language processing offers insights for modeling more than two modalities using a single modality (e.g., image or text) as an anchor and aligning others through maximizing their mutual information~\cite{imagebind, zhu2023languagebind}. However, these methods often overlook the unique information in each modality while aligning modalities, which focus exclusively on multimodal alignment in inter-view learning.
In RRL, geospatial data contain not only shared information but also distinct aspects of a region. For example, satellite imagery provides environmental context, while POI data reveals human activities. Disregarding modality-specific details during alignment may limit the effectiveness of downstream tasks.

% {\color{purple} FactorCL~\cite{factorcl} explicitly captures both task-relevant unique ($U_{x_1}$, $U_{x_2}$) and shared ($S_{x_{12}}$) information across two modalities. The objective of the unique information is defined as $U_{x_1} = I(x1; y | x2)$ (where $y$ is a task-relevant representation). This approach shows promising results in various domains, such as mortality prediction using tabular health records with sensor data.}
% {\color{purple} However, extending FactorCL to more than two modalities becomes computationally prohibitive because it requires decomposing high order shared information among multiple modalities into numerous conditional mutual information terms. Specifically, FactorCL models high order triplets ($S_{x_{123}}=\arg\max_{}I(x_1; x_2; x_3 ; y)$) and quadruplets ($S_{x_{1234}} = \arg\max_{}I(x_1; x_2; x_3 ; x_4 ;y)$), which decomposes them by the chain rule and further increases substantial computational demands.

A recent study in machine learning, FactorCL~\cite{factorcl}, introduces an information factorization approach that explicitly captures shared information ($S_{x_{12}}$) and task-relevant unique information ($U_{x_1}$, $U_{x_2}$) between two modalities, $x_1$ and $x_2$, by maximizing mutual information between modalities. 
{\color{purple}However, extending FactorCL to more than two modalities for RRL is challenging. Approximating high-order shared information requires decomposing it into a complex chain of conditional mutual information terms, which increases computational complexity.} 
% and significantly slows down training convergence.

% In practice, however, pairwise interaction often suffices to reveal key region patterns~\cite{everything}. This is because high order combinations sometimes do not introduce new information beyond what is already captured by pairwise interactions. For instance, satellite imagery and Area-Of-Interst data together may already identify an area's land function as a leisure area, and adding POI data that indicates a playground or trail would simply confirm this rather than contribute additional insights. 

% However, applying FactorCL to more than two modalities becomes computationally expensive because FactorCL requires decomposing shared information across multiple modalities into a combinatorial number of conditional mutual information terms.
% Specifically, with $m$ modalities, there are $2^m-1$ possible combinations representing shared and unique information. For instance, with three modalities ($d_1$, $d_2$, $d_3$), the objectives include the computation of individual, pairwise, and triplet sets of representations, which refer to unique ($U_{z_1}$, $U_{z_2}$, $U_{z_3}$) and shared information ($S_{z_{12}}$, $S_{z_{13}}$, $S_{z_{23}}$, $S_{z_{123}}$), a total of 7. With four modalities, the number of shared and unique information increases to $15$ combinations. As a result, FactorCL’s complexity scales to $O(2^m)$ with the exponential increase in combinations leading to substantial computational demands. Decomposing information in FactorCL is prohibitively complex as the number of modalities grows.

% While directly adopting FactorCL in multimodal region representation learning allows for capturing shared information among more than two modalities (i.e., high-order combinations) like triplet (e.g., $S_{z_{123}}$) or quadruplets (e.g., $S_{z_{1234}}$), empirically, the complementary information between pairs of modalities often suffices to reveal key region patterns~\cite{everything}. This is because high-order combinations sometimes do not introduce new information beyond what is already captured by pairwise interactions.
% % Specifically, they demonstrate the encoders with pairwise and triplet interactions show the same coding performance and demonstrate theoretically. 
% For instance, satellite imagery and AOI data may already identify an area as a park (e.g., leisure area), and adding POI data that indicates a playground or trail would simply confirm this rather than contribute additional insights. While high-order combinations can provide supplementary details, the essential patterns are often adequately captured through pairwise interactions.

% Although directly adopting FactorCL in multimodal region representation captures shared information among more than two modalities like triplets (e.g., $S_{z_{123}}$) or quadruplets (e.g., $S_{z_{1234}}$), the complementary information between pair modalities often suffices to capture region patterns without needing additional shared information among three or more modalities, i.e., high-order combinations. 
% % Although FactorCL captures shared information among more than two modalities like triplets (e.g., $S_{z_{123}}$) or quadruplets (e.g., $S_{z_{1234}}$), focusing on pairwise interactions (e.g., $S_{z_{12}}$) often suffices to capture key patterns.
% % This approach can effectively reflect essential relationships without needing additional shared information among three or more modalities, i.e., high-order combinations. 
% While high-order combinations can provide additional details, the core insights are adequately captured through the interactions between pairs of modalities.
% For example, if satellite imagery and AOI data already identify an area as a park (e.g., leisure area), adding POI data that indicates a playground or trail does not provide new information but only confirms what is already known.


% Unlike $O(2^m)$ complexity of FactorCL, our method has a complexity of $O(m^2)$ by considering only the pairwise interactions between modalities, which substantially reduces computational costs. 

% Therefore, we propose a pairwise inter-view learning method that considers all modalities in pairs, focusing on each pair's shared information to achieve comprehensiveness and computational efficiency when fusing more than two modalities.
% Figure~\ref{intro_fig} illustrates an example of unique and shared information in pairwise inter-view learning. We represent the task-relevant unique feature as $U_{z_1}$, which captures the mutual information between $z_1$ and the task-relevant representation $z^\prime$, conditioned on other input modalities. The task-relevant shared feature, $S_{z_{13}}$, shows the shared information between $z_1$, $z_3$, and $z^\prime$, conditioned on the remaining input modality. We then decompose both $U_{z_1}$ and $S_{z_{13}}$ by considering task-relevant information and excluding task-irrelevant information. 
% Figure~\ref{intro_fig} illustrates the unique and shared pairwise inter-view learning captures task-relevant modality-specific and shared features.
% Specifically, $U_{z_1}$ represents the mutual information between the $d_1$ modality and task-relevant semantics $z^\prime$ conditioned on other input modalities. Similarly, $S_{z_{13}}$ denotes the shared information among $d_1$, $d_3$, and $z^\prime$ conditioned on the other remaining input modality. 

% Building on this pairwise inter-view learning, we propose a multimodal region representation approach, \modelnamex\footnote{\modelname refers to \textbf{C}r\textbf{O}ss m\textbf{O}dal \textbf{K}nowledge \textbf{I}njected \textbf{E}mbedding}\logov with two primary goals.
% First, we aim to capture region representations of a modality that are distinctive across regions through intra-view contrastive learning by maximizing discrepancies between regions, inspired by~\cite{tkde,li2024urban}. 
% Second, we leverage pairwise inter-view learning to capture task-relevant information that spans both modality-specific and shared features across modalities.
% We then optimize intra and pairwise inter-view learning jointly and generate a comprehensive multimodal region representation. 
% To demonstrate \modelnamex, we use POI data, AOI data, satellite imagery, and building footprint to learn region vectors and evaluate the representations using several downstream tasks, such as population density, crime rate, greenness score prediction, and land use classification.

To address these challenges, we propose a novel multimodal region representation learning approach, \modelnamex\footnote{\modelname refers to \textbf{C}r\textbf{O}ss m\textbf{O}dal \textbf{K}nowledge \textbf{I}njected \textbf{E}mbedding}\logov, to effectively model multimodal geospatial data.\footnote{This work focuses on the scenarios where the number of modalities is larger than 2.} We first extend FactorCL to accommodate more than two modalities for RRL. 
{\color{purple} We observe that pairwise shared information without considering conditional mutual information naturally captures high-order dependencies. This could be because such cross-modal interactions inherently encode relationships across modalities, which makes explicit conditioning on an additional modality unnecessary. 

Moreover, estimating conditional mutual information requires learning distributions conditioned on the remaining modality, which introduces computational complexity. This conditioning step forces the model to learn fine-grained dependencies that may not always contribute meaningfully to representation learning, particularly if the conditioned modality is already entangled with the existing dependencies among the other modalties. 
}
% {\color{purple} We observe that high-order shared information across multiple modalities often provides limited benefits or can even degrade performance for downstream tasks. This could be because such cross-modal intersected information is too weak to influence the task performance, and it introduces complexity that negatively affects learning. }

% FactorCL extends: S12 = I(x1; x2; y | x3)
% CooKIE: S12 = I(x1; x2; y) 

Motivated by this finding, \modelname introduces a new inter-view learning strategy that focuses on capturing (1) task-relevant unique information from each modality, and {\color{purple} (2) low-order (pairwise) shared information, which naturally captures high-order dependencies. } %(2) low-order (pairwise) conditional shared information. 
Figure~\ref{intro_fig} illustrates the decomposition process of learning unique and pairwise shared information with three modalities. This reduced-order learning strategy not only minimizes the influence of uninformative information but also lowers the computational complexity. 
In addition, \modelname incorporates intra-view learning to pretrain the encoder for each modality to maximize inter-region discrepancies, providing a robust initialization for further training. To demonstrate \modelnamex, we utilize diverse geospatial datasets---POI data, AOI data, satellite imagery, and building footprints---to learn region representations. We then evaluate these representations on several downstream tasks in New York City (NYC), United States, and Delhi, India, including population density estimation, crime rate prediction, greenness score assessment, and land use classification.

% This part below is not yet updated!!!!!!!!!!!!!! ===========================================
The contributions of our paper are as follows,
\begin{itemize}
    \item We propose \modelnamex, a region representation learning approach, to learn region embeddings from an arbitrary number of modalities.
    \item \modelname captures both task-relevant shared and unique information in pairwise inter-view learning. We evaluate \modelname by predicting several downstream tasks such as population density, crime rate, land use function, and greenness in NYC and Delhi. % , where geospatial data distributions vary.
    \item We demonstrate that \modelname has a lower computational complexity compared to a existing method. 
    % reducing the complexity from $O(2^m)$ to $O(m^2)$ with $m$ modalities.
\end{itemize}

% Need to update the figure & explanation:: z -> x 
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/intro_.png}
    \caption{{\color{red}FIG WILL BE UPDATE: }Unique information and shared information in pairwise interaction among three input modalities and task-relevant semantics $z^\prime$, where $z$ is a representation of $x$ modality.}
    \label{intro_fig}
\end{figure}



% 1. you propose a region representation learning method to learn from arbitrary number of modalities
% 2. the learnt representations can capture ... and can do well in predicting regional tasks
% 3. it has low computational complexity (e.g., reducing how many terms, not saying you are others extension)

==> sections/background.tex <==
{\color{orange}\section{Backgrounds $\rightarrow$ \textbf{Appendix??}} }

\subsection{Factorized Contrastive Learning (FactorCL)}\label{factorcl:background}
FactorCL~\cite{factorcl} demonstrates how to capture task-relevant shared and unique information between two modalities by decomposing task-relevant and task-irrelevant semantics in both supervised and self-supervised learning. 
For shared information between modalities $i$ and $j$ ($S_{x_{ij}}$), FactorCL learns task-relevant shared information by maximizing lower bound of $I_{NCE}(x_i, x_j)$~\cite{oord2018representation} and removes task-irrelevant information by minimizing upper bound of the conditional mutual information, $-I_{CLUB}(x_i, x_j | x_i^\prime, x_j^\prime)$~\cite{clubloss}, where $x^\prime$ refers to an augmentation of $x$ (More detail restates in Section~\ref{bg:aug}). For unique information ($U_{x_{i}}$), FactorCL captures task-relevant unique feature by maximizing lower bound of $I_{NCE}(x_i, x_i^\prime)$ while removing non-unique feature by minimizing upper bound of $-(I_{CLUB}(x_i, x_j)$ $- I_{NCE}(x_i; x_j | x_i^\prime, x_j^\prime))$. 
Specifically, $I_{NCE}$ (i.e., InfoNCE loss) for conditional mutual information is defined as: 
\begin{align} \label{eq:infoNCE}
    &I_{NCE}(x_i;x_j|x_i^{\prime};x_j^{\prime})  \nonumber \\
    & \!\!\!\!\!\!\!\!=\mathbb{E}_{p(x_i^{\prime}, x_j^{\prime})} 
    \!\!\left[ \mathbb{E}_{\substack{x_i, x_j^{+}\sim p(x_i, x_j^{+} | x_i^\prime, x_j^\prime) \\ x_j^- \sim p(x_j^- | x_i^\prime, x_j^\prime)}}\!\left[ \log\frac{\exp(f(x_i, x_j^{+}, x_i^{\prime}, x_j^{\prime}))}{\sum \exp(f(x_i, x_j^{-}, x_i^{\prime}, x_j^{\prime}))}\right]\right],
\end{align}
{\color{purple}where $x_j^{+}$ is augmentation pair of $x_j$ and $x_j^{-}$ is the other samples of the same modality of $x_j$ given knowledge of $x_i^{\prime}$ and $x_j^{\prime}$, and $f(\cdot)$ is an encoder.
% where $x_i^{\prime}$ and $x_j^{\prime}$ are the positive augmentation pair of $x_i$ and $x_j$ modality, $x_j^{+}$ and $x_j^{-}$ are the positive (e.g., an augmented data sample of the region) and negative augmentations (e.g., the same modality sample of other regions) of $x_j$ given knowledge of $x_i^{\prime}$ and $x_j^{\prime}$, $f(\cdot)$ is an encoder, and 
The summation in the denominator is with respect to negative samples $x_j^-$. We note that $x_j^{\prime}$ and $(x_i,x_j^+)$ are distributed according to $x_j^{\prime} \sim p(x_j^{\prime})$ and $(x_j,x_j^{\prime})\sim p(x_i, x_j^+|x_i^{\prime}, x_j^{\prime})$ (for more details, see~\cite[eq.~(15)]{factorcl}). Finally, the maximum mutual information can be derived by the lower bound i.e., $I(x_i; x_j) \geq -I_{NCE}(x_i; x_j)$~\cite{oord2018representation}.
}

Similarly, $I_{CLUB}$ removes task-irrelevant information by minimizing the upper bound of the mutual information between $x_i$ and $x_j$~\cite[Theorem 3.1.]{clubloss} (i.e., $I_{CLUB}(x_i; x_j) \geq I(x_i; x_j)$). CLUB loss for conditional mutual information is defined as:
\begin{align}\label{eq:club}
    & I_{CLUB}(x_i;x_j|x_i^{\prime};x_j^{\prime}) \nonumber \\
    & \! = \mathbb{E}_{p(x_i^{\prime}, x_j^{\prime})} \left[ \mathbb{E}_{x_i, x_j^{+} \sim p(x_i, x_j^{+} | x_i^\prime, x_j^\prime)} \left[f(x_i, x_j^{+}, x_i^{\prime}, x_j^{\prime})\right] \right.  \nonumber \\
    & \qquad\qquad\quad \left.- \mathbb{E}_{\substack{x_i \sim p(x_i | x_i^\prime, x_j^\prime) \\ x_j^- \sim p(x_j^- | x_i^\prime, x_j^\prime)}} \left[ f(x_i, x_j^{-}, x_i^{\prime}, x_j^{\prime}) \right] \right],
\end{align}
where $f$ refers to the same encoder used in $I_{NCE}$.

{\color{purple}
\subsection{Optimal Augmentation}\label{bg:aug}
FactorCL~\cite{factorcl} employs the \textit{optimal unimodal augmentation} assumption to capture task-relevant information without relying on labels. This assumption treats an augmented pair $x^\prime$ of the $x$ modality as a substitute for the $y$ label. This means that when all information shared between $x$ and $x^\prime$ is task-relevant, implying that the augmentation preserves task-relevant information while changing task-irrelevant information. 
\begin{align}
I(x;y) = I(x;x^\prime),
\end{align} 
ensuring that $x^{\prime}$ retains the label-relevant semantic of $x$. If an augmentation discards essential semantic features (e.g., via aggressive cropping), then the shared information drops below the label signal, yielding $I(x; x^{\prime}) < I(x; y)$. Hence, FactorCL proposes \textit{optimal unimodal augmentation} that preserves all necessary semantics. This augmentation is built upon the \textit{optimal representation of a task}~\cite{tian2020makes}, which indicates that for a task $\tau$ aiming to predict a semantic label $y$ from input $x$, an encoder
\begin{align} 
f(x;\theta): x_1, x_2, \ldots, x_n &\rightarrow z_1, z_2, \ldots, z_n, 
\end{align}
produce a \textit{minimal sufficient statistic} $z$ that maintains all label-relevant information while discarding extraneous details. Consequently, by treating $x^{\prime}$ as a valid proxy for $y$, \modelname can learn a representation $z$ that is both sufficient and minimal for the downstream prediction task. 
}

==> sections/preliminary.tex <==
% \section{Problem Statement}
% \begin{definition}[Urban regions] A city can be divided into distinct regions, defined as $\mathcal{U} = \{ u_1, ... , u_n\}$, where $n$ is the number of regions. We use census tracts and ward-level boundaries as partitions.
% \end{definition}

% \begin{definition}[Urban attributes]
% A region is characterized by a set of modalities, denoted as $\mathcal{X} = \{x_1,..., x_m\}$, where $m$ is the number of modalities and $x_i$ represents $i$-th modality, such as POI, AOI, or satellite imagery.
% \end{definition}

% % \begin{problemstate}[Urban region representation learning]
% \textbf{Problem Statement (Urban region representation learning).}
% Given a set of regions $\mathcal{U}$, we aim to learn representations from the modalities $\mathcal{X}$. The learned region embeddings are denoted as $E = \{ e_1, ..., e_n\}$, where $e_i \in \mathbb{R}^k$ represents the embedding for region $i$, and $k$ is the embedding dimension.
% % \end{problemstate}
